The Limits of Optimal Pricing in the Dark

A ubiquitous learning problem in today's digital market is, during repeated interactions between a seller and a buyer, how a seller can gradually learn optimal pricing decisions based on the buyer's past purchase responses. A fundamental challenge of learning in such a strategic setup is that the buyer will naturally have incentives to manipulate his responses in order to induce more favorable learning outcomes for him. To understand the limits of the seller's learning when facing such a strategic and possibly manipulative buyer, we study a natural yet powerful buyer manipulation strategy. That is, before the pricing game starts, the buyer simply commits to "imitate" a different value function by pretending to always react optimally according to this imitative value function. We fully characterize the optimal imitative value function that the buyer should imitate as well as the resultant seller revenue and buyer surplus under this optimal buyer manipulation. Our characterizations reveal many useful insights about what happens at equilibrium. For example, a seller with concave production cost will obtain essentially 0 revenue at equilibrium whereas the revenue for a seller with convex production cost is the Bregman divergence of her cost function between no production and certain production. Finally, and importantly, we show that a more powerful class of pricing schemes does not necessarily increase, in fact, may be harmful to, the seller's revenue. Our results not only lead to an effective prescriptive way for buyers to manipulate learning algorithms but also shed lights on the limits of what a seller can really achieve when pricing in the dark.

==> backup - Copy/characterization.tex <==
\section{The Equilibrium of \name{} under Linear Pricing, and    Implications}\label{sec:characterization}
In this section, we characterize  the  equilibrium of    \name{}  under  linear pricing schemes, i.e., $\P = \P_L=\{p: p(\bvec{x}) = \bvec{p} \cdot \bvec{x} \text{ for some } \bvec{p}\in \mathbb{R}^d_{+} \}$  consists of all linear pricing functions. A linear pricing function is determined by a non-negative price vector   $\bvec{p}\in \mathbb{R}^d_{+}$. To distinguish \emph{functionals} from \emph{vector variables},  we will  use $P_L= \{  \bvec{p}:  \bvec{p}\in \mathbb{R}^d_{+}\}$ to denote the set of all  possible non-negative price vectors so that each  $\bvec{p} \in P_L$ uniquely corresponds to a linear pricing function in $\P_L$.   Under linear pricing, the equilibrium in Def. \ref{def:equ}  denoted by $(u^*, \bvec{p}^*, \bvec{x}^*)$ is characterized by Eq. \eqref{eq:equilibrium-def} where $\P = \P_L$.
%\vspace{-2mm}
%the following formulation:
%\begin{eqnarray}\nonumber  
%&& u^* = \argmax_{u  \in \C}  [  v(\bvec{x}^*) -  \bvec{p}^* \cdot \bvec{x}^*  ],   \\ \label{eq:equilibrium-def-linear} 
%\text{ where } &&   \bvec{p}^* = \argmax_{\bvec{p}  \in P_L}  [ \bvec{p} \cdot  \bvec{x}^*  - c(\bvec{x}^*) ],  \\  \nonumber 
%\text{ where }  &&  \bvec{x}^* = \argmax_{\bvec{x} \in X} \big[ u^*(\bvec{x}) - \bvec{p}^* \cdot  \bvec{x} \big] 
%\end{eqnarray} 
 
%\mh{This section characterizes  the equilibrium of the  \name{} problem: what any “effective” learning algorithm (Def. \ref{def:T-effective}), e.g., the algorithm in \cite{roth2016watch}, will learn when being used against a strategically responding buyer}. 

% \begin{wrapfigure}{r}{0.25\textwidth}
%	\centering
%	\includegraphics[width=0.25\textwidth]{figures/general_cost2.pdf}
%	\caption{Illustration of $p^*$ in Theorem \ref{thm:characterization}.  }
%	\label{fig:c_and_u}
%\end{wrapfigure}

%\vspace{-2mm}
Even with linear pricing,  this is still a very challenging \emph{tri-level functional} optimization problem since $u^*$ is a function  chosen from the set of all possible functions from $X$ to $\RR_+$, denoted by set $\C$.  A first thought one might have is: why doesn't the buyer simply imitate $u^*(\bvec{x}) = c(\bvec{x})$. We will see later that this is  not ---  in fact far from being --- optimal since it   makes the game zero-sum and the seller will pick a price that guarantee 0 revenue, e.g., a price of $\infty$. This leads the trade to happen at 0 production, which  is clearly not optimal for the buyer. The optimal $u^*$ should provide some incentive for the seller to produce some amount $\bvec{x}^*$ that is  in some sense the best for the buyer. We will provide two concrete examples in the next section in Figure \ref{fig:one-dimensional-characterization2}.   

The main result of this section is the following  characterization for the equilibrium of \name{}. This general characterization does not depend on any specific property about function $v(\bvec{x}), c(\bvec{x})$.  

%\begin{theorem}
\begin{restatable}{restatethm}{primethmcharacterization}
\label{thm:characterization}In the  equilibrium of \name{} under linear pricing, the optimal buyer imitative  value function $u^*$  can w.l.o.g. be written as the following concave function parameterized by  production amount $ \bvec{x}^*\in X$ and a real value $p^* \in \RR_+$: 
	%	\begin{equation}\label{eq:optimal-format}
	%		u^*(\bvec{x}) = 
	%		\begin{cases}
	%			\bvec{p}^* \cdot \bvec{x}  & \text{if $\bvec{x} \in X(x^*)$} \\
	%			\bvec{p}^* \cdot \bvec{x}^* & \text{if $\bvec{x} \notin X(\bvec{x}^*)$}
	%		\end{cases}
	%	\end{equation}
	%    \qd{ 
	\begin{equation} \label{eq:optimal-format}
	u^*(\bvec{x}) =p^*  \cdot \min \{ \frac{x_1}{x^*_1}, \cdots \frac{x_d}{x^*_d}, 1\}   
	% \sum_{i\in d^{\bvec{x},\bvec{x}^*}_{\leq}} p^*_i x_i + \sum_{j\in d^{\bvec{x},\bvec{x}^*}_{>}} p^*_j x^*_j
	\end{equation}
	%}
	where 
	\begin{equation}\label{eq:optimal-xp}
\bvec{x}^* = \arg \max_{\bvec{x} \in X} \big[  v(\bvec{x}) - \sup_{\alpha \in [0,1)} \frac{  c( \bvec{x}) -c(\alpha \bvec{x}) }{1 - \alpha} \big] \quad \text{ and } \quad p^* =  \sup_{\alpha \in [0,1)} \frac{  c( \bvec{x}^*) -c(\alpha \bvec{x}^*) }{1 - \alpha} 
	\end{equation}
%	$(\bvec{x}^*, p^*)$    is the optimal solution to the following optimization program  with variables $p, \bvec{x}$:
%	\begin{lp}\label{lp:buyer-simple-thm}
%		\maxi{ v(\bvec{x}) - p  }
%		\st 
%			\qcon{p  - c( \bvec{x}) \geq \alpha  \cdot p - c(\alpha \bvec{x})}{   \alpha \in [0,1] } 
%					\con{ \bvec{x}  \in  X, p \in \RR } 
%	\end{lp} 
	
	Moreover, under imitative value function $u^*(\bvec{x})$,  
	\begin{enumerate}
		\item For any   vector $\lambda \in \Delta_d$ in the $d$-dimensional simplex,  the linear pricing scheme with  price vector   $\bvec{p}^* =  (\lambda_1  \frac{p^*}{x_1^*}, \lambda_2   \frac{p^*}{x_2^*}, \cdots, \lambda_d   \frac{p^*}{x_d^*})$ is optimal for $u^*$. 
		%Any of the following linear pricing schemes is optimal: fix any $i \in [d]$, the  unit price for product $i$ is $p_i^* = p^*/x_i^*$ and the unit price for product $j \not = i$ is $0$. 
		\item In any of the above optimal linear pricing schemes, the buyer's optimal  bundle response is always $\bvec{x}^*$ and the buyer payment will always equal $p^*$. 
		\item At equilibrium, the buyer surplus  is $[v(\bvec{x}^*) - p^*]$ and the seller revenue is $[p^* - c(\bvec{x}^*)]$.   
	\end{enumerate}
	%The optimal seller revenue is thus $\bvec{p}^* \cdot \bvec{x}^* - c(\bvec{x}^*) \geq 0$ and optimal buyer surplus is $v(\bvec{x}^*) - \bvec{x}^* \cdot \bvec{p}^* \geq 0$.  
%\end{restatable}
\end{restatable}
%\end{theorem}
% \begin{wrapfigure}{r}{0.3\textwidth}
%	\centering
%	\includegraphics[width=0.3\textwidth]{figures/general_cost2.pdf}
%	\caption{Illustration of $p^*$ in Theorem \ref{thm:characterization}.  }
%	\label{fig:c_and_u}
%\end{wrapfigure}
%\
%\

Note that the $u^*$ described by Equation \eqref{eq:optimal-format} may not be the unique optimal buyer imitative value function, but it is one of the optimal ones. Moreover, any optimal imitative value function will result in the same buyer surplus and seller revenue. 
%
% \begin{wrapfigure}{r}{0.3\textwidth}
%	\centering
%	\includegraphics[width=0.3\textwidth]{figures/general_cost2.pdf}
%	\caption{Illustration of $p^*$ in Theorem \ref{thm:characterization}.  }
%	\label{fig:c_and_u}
%\end{wrapfigure}
%\
%\

% \begin{wrapfigure}{R}{0.25\textwidth}
%	\centering
%	\includegraphics[width=0.25\textwidth]{figures/general_cost2.pdf}
%	\caption{Illustration of $p^*$ in Theorem \ref{thm:characterization}.  }
%	\label{fig:c_and_u}
%\end{wrapfigure}
%\
%\

{\bf Interpretation of Theorem \ref{thm:characterization}. }  Before a formal proof,  it is worthwhile to take a closer look at the characterization of the buyer's optimal imitative value function $u^*$ characterized by Theorem \ref{thm:characterization} and the special pricing problem it ultimately induces.   At a high level, the buyer has a desirable amount of products $\bvec{x}^*$ in mind, characterized by the first equation in \eqref{eq:optimal-xp}. He would pretend that his value for $\bvec{x}^*$ equals $p^*$. Moreover, the value of any production amount $\bvec{x}$ will linearly depend on the  maximum  possible coordinate-wise \emph{fraction} of $\bvec{x}^*$ that $\bvec{x}$ contains, i.e.,  the $ \min \{ \frac{x_1}{x^*_1}, \cdots \frac{x_d}{x^*_d}, 1\} $ term in $u^*$.\footnote{Notably, the format of this  value function appears to have interesting connections to the well-known   \emph{Leontief   production function}  \cite{allen1967macro} which has the format of $\min_i \{ \frac{x_i}{a_i}\}$. However, leontief functions  are used  to describe seller's production \emph{quantities} as a function of quantities of different factors with no substitutability. It is an expected surprise that similar type of \emph{value} function turns out to be   optimal for buyer's strategic manipulation.  } 
 \begin{wrapfigure}{R}{0.25\textwidth}
	\centering
	\includegraphics[width=0.25\textwidth]{figures/general_cost2.pdf}
	\caption{Illustration of $p^*$ in Theorem \ref{thm:characterization}.  }
	\label{fig:c_and_u}
\end{wrapfigure}
\
\

The $p^*$ is chosen as the largest possible \emph{slope} of the segment between $c( \bvec{x}^*)$ to $c( \alpha \bvec{x}^*)$ among all possible $\alpha \in [0,1)$ (see Figure \ref{fig:c_and_u} for an illustration in one dimension about how $p^*$ is chosen based on the cost function $c$). This is certainly a very carefully chosen value.  Note that  \[p^* =   \sup_{\alpha \in [0,1)} \frac{  c( \bvec{x}^*) -c(\alpha \bvec{x}^*) }{1 - \alpha}  \geq     \frac{  c( \bvec{x}^*) -c( \bvec{0}) }{1 - 0}  = c(\bvec{x}^*),\] which implies  non-negativity of  the seller's revenue $[p^* - c(\bvec{x}^*)]$. In fact, the seller can achieve \emph{strictly positive}  revenue if and only if the above $\geq$ is strict.  Finally, the  optimal buyer imitative value function $u^*$ leads to a special pricing problem for the seller.  Since the buyer's value is designed such that he is only interested in purchasing some fraction $r\in [0,1]$  of $\bvec{x}^*$, the seller's optimal pricing will    charge  $r p^*$ for the bundle $\bvec{x} = r \bvec{x}^*$  and this total charge $r p^*$ can be distributed \emph{arbitrarily} over the $d$ products, e.g., by charging  $\lambda_i  r p^* = \lambda_i \frac{p^*\cdot x_i}{x_i^*} $  for product $i$ where $\sum_{i=1}^d \lambda_i = 1$.  Overall, Theorem \ref{thm:characterization} fully characterized what the pricing problem is like at the equilibrium of \name{}.  
 
\begin{remark}\label{remark1}
Theorem \ref{thm:characterization} only provides a structural characterization about the equilibrium but does not imply that the equilibrium $(u^*, \bvec{p}^*, \bvec{x}^*)$ can be computed efficiently since we still need to solve the optimization problem  \eqref{eq:optimal-xp} to find the optimal $\bvec{x}^*$. As we will show later, this turns out actually to be an NP-hard problem in general. This is an interesting situation where the result reveals useful structural insights   despite  its computational intractability. 
\end{remark}  


%\begin{remark}\label{remark2}
%The proof of Theorem \ref{thm:characterization}  relies   on the concavity of imitative value functions. Without this restriction, the buyer can always obtain the largest possible surplus $\max_{\bvec{x} \in X} [v(\bvec{x}) - c(\bvec{x})]$ through, e.g.,  the following (not realistic) imitative value function: let $\bar{\bvec{x}} = \arg \max_{\bvec{x} \in X} [v(\bvec{x}) - c(\bvec{x})]$ and imitate value function $u$ such that $u(\bvec{x}) = c(\bar{\bvec{x}})$ for any $\bvec{x} \geq \bar{\bvec{x}}$ entry-wise and $u(\bvec{x}) = 0$ otherwise.  This function is not even continuous, though it can induce the trade to happen at $\bar{\bvec{x}}$ with payment  $c(\bar{\bvec{x}})$. % This illustrates that if the restriction to buyer's imitative value function 
%\end{remark}  

% This theorem provides a characterization about how a   buyer will strategically reveal his preference to a learning seller and what the seller will learn at the ex-post equilibrium, under our behavorial assumption on both agents. One might wonder that, knowing the buyer may be imitating a different value function, why the seller does not design a learning mechanism that takes the buyer's strategic behaviors into account. This is because any such learning mechanism will necessarily violate effectiveness assumption,  and thus is ruled out by our assumption. From this perspective,  Theorem \ref{thm:characterization} can   be  alternatively interpreted as a characterization of what any  learning algorithm that is effective for honest buyers (e.g., the algorithm of \cite{roth2016watch})  will learn when being used against a strategic buyer.  We leave it as an intriguing open question to analyze what the equilibrium would be like in the full generality of this dynamic game.    


%\subsection*{Proof of Theorem \ref{thm:characterization}}
\vspace{-2mm}
\begin{proof}[ Proof Sketch of Theorem \ref{thm:characterization}.]  The  proof of Theorem \ref{thm:characterization} is somewhat involved. We give a sketch here and defer formal arguments to Appendix \ref{app_sec:proof-characterization}.   The most challenging part is to find the optimal function $u^* \in \C$, which is a \emph{functional optimization} problem.    Standard optimization analysis only apply to programs with vector variables, while not functional variables. To overcome this challenge, our proof has two major steps. First, 
% This is divided into two steps. First,  we   show that it is without loss of generality to consider only concave value function $u(\bvec{x})$ to imitate. This proof is built upon a classical mathematical result about the existence of a concave function $u: \RR^d \to \RR$ to fit any given multi-valued function $\bvec{p}: X \to \RR^d$ in the \emph{first order} sense: $\partial u(\bvec{x}) = \bvec{p}(\bvec{x})$. 
 we  argue that the concave functions of the specific format as in Equation \eqref{eq:optimal-format} would suffice to help the buyer to achieve optimality. This effectively    reduce the functional optimization problem to a variable optimization problem since any function of  Format  \eqref{eq:optimal-format} can be characterized by $d+1$ variables. Second, we then analyze the variable optimization problem we get and prove characterization of its optimal solutions. The first step is the most involved part and uses a significant amount of convex analysis. Such complication comes from the reasoning over the tri-level optimization problem  \eqref{eq:equilibrium-def}. Tri-level optimization is generally highly intractable  \cite{ben1990computational}  --- indeed, as we will show later,  computing the equilibrium $(u^*, \bvec{p}^*, \bvec{x}^*)$ is NP-hard in general.  Nevertheless, our analysis was able to bypass the difficulty by leveraging the special structure of the pricing problem and leads to a clean and useful characterization for the structure of the equilibrium.  
 
 
  A crucial intermediate step  is the following characterization for a slightly simpler version of the question. That is,  fixing any bundle $\bar{\bvec{x}} \in X$, which imitative value function $u(\bvec{x})$ will maximize the utility of the \emph{buyer} with true value function $v(\bvec{x})$, subject to that the optimal buyer purchase response under $u(\bvec{x})$  is $\bar{\bvec{x}}$? Fortunately,  this question indeed admits a succinct characterization as shown below.
  %as we show in Lemma \ref{lem:characterization-fix-y0}. % We adopt the following notation: for any $\bvec{x} , \bar{\bvec{x}}  \in X \subseteq \mathbb{R}^d$, let $d^{\bvec{x}, \bar{\bvec{x}} }_{\leq} = \{i |x_{ i} \leq \bar{x}_i \}$ denote the set of indexes with $x_{i} \leq \bar{x}_{i}$ and $d^{\bvec{x} , \bar{\bvec{x}}}_{>} = \{i |x_{ i} > \bar{x}_{i} \}$ is the complement of  $d^{\bvec{x},  \bar{\bvec{x}}}_{\leq} $. 
 %for any $\bar{\bvec{x} } \in X$, let $X(\bar{\bvec{x}}) = \{ \bvec{x} \in X: \bvec{x} \leq \bar{\bvec{x}} \}$ be the set $X$ truncated by  $\bvec{x} \leq \bar{\bvec{x}}$ (entry-wise smaller)  \mh{For any $\bvec{x}_1, \bvec{x}_2 \in X \subseteq \mathbb{R}^d$, let $d^{\bvec{x}_1, \bvec{x}_2}_{\leq} = \{i |x_{1i} \leq x_{2i} \}$ and $d^{\bvec{x}_1, \bvec{x}_2}_{>} = \{i |x_{1i} > x_{2i} \}$. }.   
 %\vspace{-2mm}
 
 \begin{restatable}{lemma}{primelemmacharacterizationfixy}
 %\begin{lemma}
 	\label{lem:characterization-fix-y0}%[Optimal Imitative Valuation Function w.r.t. Buyer Bundle $\bar{\bvec{x}}$] 
 	For any bundle $\bar{\bvec{x}} \in X$, the optimal buyer imitative   value function 
 	$\bar{u}(\bvec{x})$, subject to that the resultant optimal buyer purchase response is  bundle $\bar{\bvec{x}}$, can without loss of generality have the following piece-wise linear  concave function format, parameterized by a real number $ \bar{p} \in \RR$: 
 	\begin{equation} \label{eq:optimalformat_lem0}
 		%\bar{u}(\bvec{x}) = \sum_{i =1}^d  \bar{p}_i  \min  \{ x_i,   \bar{x}_i \} 
 		\bar{u}(\bvec{x})  = \bar{p} \cdot \min \{ \frac{x_1}{\bar{x}_1}, \cdots \frac{x_d}{\bar{x}_d}, 1\}  
 	\end{equation}
 	%\mh{\begin{equation} \label{eq:optimalformat_mh}
 	%	\bar{u}(\bvec{x}) =\begin{cases}
 	%		\bar{\bvec{p}} \cdot \bvec{x}  & \text{if $\bvec{x} = \alpha \cdot \bar{\bvec{x}}, \alpha \in [0,1]$} \\
 	%		-\infty & \text{otherwise}
 	%	\end{cases}
 	%\end{equation}}
 	%	\todo{simplified notation, please check}
 	%\mh{One generalization of this equation \eqref{eq:optimalformat1_new} is 
 	%\begin{equation} \label{eq:optimalformat1_gen}
 	%	\bar{u}(\bvec{x}) =\begin{cases}
 	%		\bvec{x} \cdot \frac{ \bvec{\bar{x}}\cdot \bar{\bvec{p}} \cdot \bvec{\bar{x}}  }{\|\bvec{\bar{x}}\|^2}& \text{if $\bvec{x} \cdot \bvec{\bar{x}} \leq \|\bvec{\bar{x}}\|^2$ } \\
 	%		\bar{\bvec{p}} \cdot \bvec{\bar{x}}  & \text{otherwise}
 	%	\end{cases}\end{equation}. Note that $\nabla \bar{u}(\bvec{x}) = \frac{ \bvec{\bar{x}}\cdot \bar{\bvec{p}} \cdot \bvec{\bar{x}}  }{\|\bvec{\bar{x}}\|^2}$ if $\bvec{x} \cdot \bvec{\bar{x}} \leq \|\bvec{\bar{x}}\|^2$. Therefore, if $\bar{p}_i=\bar{p}_j$ and $\bar{x}_i=\bar{x}_j$ for any $i\neq j$, we'll have $\nabla \bar{u}(\bvec{x}) = \bvec{\bar{p}}$. Hence, my previous counter-example for proving $\nabla u^*(\bvec{x}') \cdot \bvec{x}' < \nabla \bar{u}(\bvec{x}') \cdot \bvec{x}'=\bvec{\bar{p}}\cdot \bvec{x}'$ when $\bvec{x}'$ is element-wise smaller than $\bvec{\bar{x}}$ which also absolutely satisfies $\bvec{x} \cdot \bvec{\bar{x}} \leq \|\bvec{\bar{x}}\|^2$ can be used again. Recall the counter example is $u^*(\bvec{x}) = \sqrt{x_1 \cdot x_2}$ and $\bvec{\bar{x}} = [9,9]$ and $\bvec{x}'=[4,1]$.}
 	%	\begin{equation} \label{optimalformat1}
 	%	\bar{u}(\bvec{x}) = 
 	%	\begin{cases}
 	%	\bar{\bvec{p}} \cdot \bvec{x}  & \text{if $\bvec{x} \in X(\bar{\bvec{x}})$} \\
 	%	\bar{\bvec{p}} \cdot \bar{\bvec{x}} & \text{if $\bvec{x} \notin X(\bar{\bvec{x}})$}
 	%	\end{cases}
 	%	\end{equation}
 	%	\mh{	\begin{equation} \label{optimalformat1}
 	%			\bar{u}(\bvec{x}) = \sum_{i\in d^{\bvec{x},\bar{\bvec{x}}}_{\leq}} \bar{p}_i x_i + \sum_{j\in d^{\bvec{x},\bar{\bvec{x}}}_{>}} \bar{p}_j \bar{x}_j
 	%	\end{equation}}
 	where $\bar{p}  \in \RR$  is the solution to the following linear program (LP):
 	\begin{lp*} \label{lp:optimalformat_lemm}
 		\maxi{ v(\bar{\bvec{x}}) - p   }
 		\st 
 		\qcon{p - c(\bar{\bvec{x}}) \geq \alpha  \cdot p - c(\alpha \bar{\bvec{x}})}{   \alpha \in [0,1] }
 	\end{lp*}
 \end{restatable}
 %\end{lemma}
\vspace{-6mm}
\end{proof} 

%\subsection*{Proof Step 1: Sufficiency of Imitating a Concave Value Function}
%We start with a classical mathematical lemma  due to Rockafellar \cite{rockafellar1966characterization,rockafellar1970maximal}. Specifically, let $\bvec{p}(\bvec{x})$ be a general one-to-many multi-valued function from $X\subseteq \RR^d$ to $\RR^d$. The notation  $\bvec{p},\bvec{x}$ are intentional as they will be corresponding exactly to the price vector and purchase bundle in our problem.  The following lemma characterizes when it is possible to find a concave function $u$ to ``fit'' the   function $\bvec{p}(\bvec{x})$ in the first-order sense. 
%\begin{lemma}[\cite{rockafellar1966characterization,rockafellar1970maximal}]\label{lem:concave-exists}
% Given any one-to-many multi-valued function $\bvec{p}(\bvec{x}): X \to \RR^d$,  there exists a concave function $u$ such that its set of super-gradients satisfies $\partial u(\bvec{x}) = \bvec{p}(\bvec{x})$ for any $\bvec{x} \in X$ \emph{if and only if} $\bvec{p}(\bvec{x})$ satisfies the following \emph{cyclically monotone} property\footnote{It is clear here now that why the mapping is required to be generally one-to-many. This is because the super-gradients may not be unique. Note that the equality $\partial u(\bvec{x}) = \bvec{p}(\bvec{x})$ means the set of super-gradietns equal the set $\bvec{p}(\bvec{x})$. }: for any finite sequence $\bvec{x}_1, \cdots, \bvec{x}_T$ and corresponding  value sequence $\bvec{p}_1, \cdots, \bvec{p}_T$  where $\bvec{p}_t \in \bvec{p}(\bvec{x}_t)$ we have  \begin{equation}
%  \bvec{x}_1\cdot  \bvec{p}_1 + \cdots + \bvec{x}_T\cdot  \bvec{p}_T \leq   \bvec{x}_1\cdot  \bvec{p}_2  + \cdots + \bvec{x}_{T-1} \cdot  \bvec{p}_T +  \bvec{x}_{T} \cdot  \bvec{p}_1. 
% \end{equation} 
%\end{lemma} 
%
%We  leverage Lemma \ref{lem:concave-exists} to prove that it is without loss of generality for the buyer to imitative a concave value function. Let $(u^*, \bvec{p}^*, \bvec{x}^*)$ be any equilibrium of a given \name{} problem where $u^*$ is not necessarily concave. We show that there exists some \emph{concave} $\bar{u}$ such that $(\bar{u}, \bvec{p}^*, \bvec{x}^*)$  is also an equilibrium.  In fact, we prove a stronger result. That is,  there exists a concave value function $\bar{u}$ which will   lead to exactly the same buyer purchase response for \emph{any} seller price vector $\bvec{p}$. More formally, $  \argmax_{\bvec{x} \in X} \big[ u^*(\bvec{x}) - \bvec{p} \cdot  \bvec{x} \big]  = \argmax_{\bvec{x} \in X} \big[ \bar{u}(\bvec{x}) - \bvec{p} \cdot  \bvec{x} \big]  $ for any $\bvec{p}$.  Therefore, if the buyer were to imitate value function $\bar{u}$, it will not change his best response bundle $\bvec{x}^*$ to any seller price, and thus will not change the seller's optimal price $\bvec{p}^*$ neither  changing his utility $[  v(\bvec{x}^*) -  \bvec{p}^* \cdot \bvec{x}^*  ]$. So $(\bar{u}, \bvec{p}^*, \bvec{x}^*)$   will be an equilibrium as well. 
%
%Given any (not necessarily concave) function $u^*$, let us define a general multi-valued function $ \bvec{x}(\bvec{p}) =   \argmax_{\bvec{x} \in X} \big[ u^*(\bvec{x}) - \bvec{p} \cdot  \bvec{x} \big]$, which represents buyer's optimal response bundle\footnote{If there are multiple best responses, $\bvec{x}(\bvec{p}) $ can be the set of all optimal response bundles } as a function of any price vector  $\bvec{p}$. We then take the inverse of this function, denoted as $\bvec{p} (\bvec{x})$.  Note that $\bvec{p} (\bvec{x})$ is also a general one-to-many multi-valued function. For any $\bvec{x}$, $\bvec{p}(\bvec{x})$ is the set of price vectors under which $\bvec{x}$ is the optimal bundle. 
%
%We  now show that the  $\bvec{p} (\bvec{x})$ defined above satisfies the cyclically monotone property stated in Lemma \ref{lem:concave-exists}.  Take any finite sequence $\bvec{x}_1, \cdots, \bvec{x}_T$ and let $\bvec{p}_t \in \bvec{p}(\bvec{x}_t)$ by an optimal price vector under which $\bvec{x}_t$ is an optimal response bundle. Therefore, by definition, we have  (let $\bvec{x}_{0} = \bvec{x}_{T}$)
%$$
%  u^*(\bvec{x}_t) - \bvec{p}_t \cdot  \bvec{x}_t   \geq   u^*(\bvec{x}_{t-1}) - \bvec{p}_t \cdot  \bvec{x}_{t-1}, \forall  t=1, \cdots, T
%$$ 
%Summing over all the above equations over $t$, we obtain
%\begin{eqnarray*}
%	\sum_{t=1}^T \big[  u^*(\bvec{x}_t) - \bvec{p}_t \cdot  \bvec{x}_t  \big] & \geq &  \sum_{t=1}^T \big[  u^*(\bvec{x}_{t-1}) - \bvec{p}_t \cdot  \bvec{x}_{t-1} \big] =  \sum_{t=1}^T  u^*(\bvec{x}_{t}) - \sum_{t=1}^T  \bvec{p}_t \cdot \bvec{x}_{t-1}. 
%\end{eqnarray*}
%This implies  the cyclically monotone property   $	 	\sum_{t=1}^T   \bvec{p}_t \cdot  \bvec{x}_t    \geq    \sum_{t=1}^T  \bvec{p}_t \cdot \bvec{x}_{t-1}.  $,\mh{$\leq$} as desired. By Lemma \ref{lem:concave-exists}, we can find a concave function $\bar{u}$ such that $\partial \bar{u}(\bvec{x}) = \bvec{p}(\bvec{x})$.  For such a value function, we have  $ \bvec{x} =  \argmax_{\bvec{x}'  \in X} \big[ \bar{u}(\bvec{x}') - \bvec{p} \cdot  \bvec{x}' \big]$  for any   $\bvec{p} \in \partial \bar{u}(\bvec{x})  = \bvec{p}(\bvec{x})$ due to the super-gradient property:  
%$$ \forall \bvec{x}',  \bar{u}(\bvec{x}) -  \bar{u}(\bvec{x}') \geq   \bvec{p} \cdot  [ \bvec{x} -   \bvec{x}']  \quad  \text{ or equivalently } \quad  \forall \bvec{x}',  \bar{u}(\bvec{x}) - \bvec{p} \cdot  \bvec{x} \geq \bar{u}(\bvec{x}') - \bvec{p} \cdot  \bvec{x}'.$$
%Therefore, the buyer will have the same optimal responses  under value function $u^*$ and $\bar{u}$, as desired.  
%
%
%
%
%
% 


%\subsection*{Formal Proof} 

 


%Therefore,  the problem of characterizing the ex post equilibrium of \name{} boils down to characterizing the optimal \emph{imitative value function}  $u^*$ that the buyer should pretend to have.  Our main result in this section is the characterization of $u^*$.\footnote{ One might wonder why the buyer does not simply report $u(\bvec{x}) = c(\bvec{x})$. We will show later  this is  not ideal since it  makes the game zero-sum and will lead the trade to happen at 0 production, which clearly is not good for the buyer. See Figure \ref{fig:one-dimensional-characterization2} later for concrete examples.}    We will use the following notation: for any $\bvec{x}^* \in X$, let $X(\bvec{x}^*) = \{ \bvec{x} \in X: \bvec{x} \leq \bvec{x}^* \}$ be the set $X$ truncated by  $\bvec{x} \leq \bvec{x}^* $ (entry-wise smaller).   


% As a consequence, this reduces the \name{} problem to the following  single-round \emph{Pricing via Value Elicitation} problem. 
%
%\begin{definition}\label{def:vep}[Pricing via Value Elicitation (PVE)]
%	In PVE, the seller first asks the buyer  to report  concave value function $u(\bvec{x})$ and then outputs the price that maximizes her profit against $u(\bvec{x})$. The buyer best responds according to {imitative value function} $u(\bvec{x})$, as required by imitative strategies.
%\end{definition}
%The  buyer's response strategy is now summarized into the report of a strategically chosen $u(\bvec{x})$. 






==> backup - Copy/concave.tex <==
\section{The Risk of Over-exploiting Buyer's Incentives}\label{sec:nonlinear-pricing}
To counteract the buyer's strategic manipulation, one of the most  natural approaches  is perhaps to use a  richer or more powerful  class of pricing schemes, as opposed to  only using linear pricing.  Such additional power of pricing will always increase the revenue when facing an  honest buyer. Unfortunately, however, we show that it   does not necessarily help in the presence of buyer manipulation --- in fact, the seller may suffer the risk of \emph{over-exploiting the buyer's incentives} so that it becomes easier for the buyer to manipulate.  This phenomenon is similar in spirit to the \emph{overfitting} phenomenon in machine learning. That is,   using a richer hypothesis class does not necessarily reduce the testing error, though it does reduce the training error.  We believe that our findings in this section   partially explain why simple pricing schemes like linear pricing are  preferred in reality.   %Our result illustrates an analogous message in optimal pricing against deceptive buyers ---   using a richer class of pricing scheme will not necessarily increase the seller's revenue in the presence of buyer manipulations, though it does always increase the revenue when facing a honest buyer. 

We first prove that the strictly more general class of  \emph{concave} pricing schemes can never do better for the seller than the (much) restricted class of linear pricing. In fact, surprisingly,  the equilibrium of \name{} under concave pricing turns out to be exactly the same as the equilibrium under linear pricing. %Therefore, the additional power of the pricing schemes does not bring any help to the seller's revenue in presence of buyer manipulations.  
This time, our proof utilizes  a crucial observation that under concave pricing, the tri-level optimization problem of \name{}  can be reduced to solving a bi-level optimization problem (in particular, FOP \eqref{lp:optimal_deception_concave_pricing}). Recall that the proof of Theorem \ref{thm:characterization}  also reduces the tri-level FOP to a bi-level FOP through a characterization about the price and optimal buyer bundle in Lemma \ref{lem:optimalpricing}.  However,    Lemma \ref{lem:optimalpricing} does not hold any more  if   the seller uses the richer class of concave pricing schemes. Therefore,  the FOP \eqref{lp:optimal_deception_concave_pricing} we obtain here is different from the core FOP \eqref{lp:optimaldeception} we solve in the proof of Theorem \ref{thm:characterization}. Nevertheless, through careful convex analysis, we are able to show  that the optimal solution to FOP \eqref{lp:optimal_deception_concave_pricing} also admits an optimal solution of similar structure  as  characterized by Theorem \ref{thm:characterization}.  

%Specifically, we consider the strictly more general class of  \emph{concave} pricing schemes. That is,  the seller's pricing function is allowed to be any concave function.  Let $\mathcal{P}_C$ denote the set of all   concave  functions that are monotone non-decreasing with $p(\bvec{0}) = 0$ for any $p \in \P_C$.  In this case, the equilibrium of \name{} can be formulated by the following functional optimization program (FOP): 
%\begin{eqnarray}\nonumber 
%&& u^* = \argmax_{u  \in \C}  [  v(\bvec{x}^*) - p^*(\bvec{x}^* ) ],   \\ \label{eq:equilibrium-concave} 
%\text{ where } &&   p^* = \argmax_{p \in \P_C}  [  p( \bvec{x}^*)  - c(\bvec{x}^*) ],  \\  \nonumber 
%\text{ where }  &&  \bvec{x}^* = \argmax_{\bvec{x} \in X} \big[ u^*(\bvec{x}) - p^*( \bvec{x} ) \big] 
%\end{eqnarray} 


% Note that FOP \eqref{eq:equilibrium-concave}  now becomes even harder to analyze since it has two functional variables $u, p$ now. For the tractability of  analysis, we assume the buyer will only imitate concave value functions, i.e.. $\C$ in FOP \ref{eq:equilibrium-concave} consists of all concave functions. This is a valid restriction because we shall prove that the  seller will be no better (and the buyer will be no worse) under the strictly  richer class of concave pricing. Therefore, if the buyer was to have more flexibility to  choose  arbitrary value functions, this conclusion still holds.  Specifically, the main result of this section is the following

\begin{restatable}{restatethm}{primethmnonlinearpricing}
 %\begin{theorem}
 	\label{thm:non_linear_pricing_eqm}
The equilibrium of  \name{}  under \emph{concave} pricing is exactly the same as the equilibrium under \emph{linear} pricing as characterized by Theorem \ref{thm:characterization}. 
\end{restatable}
 %\end{theorem}
%\vspace{-3mm}
\begin{proof}[Proof Sketch of Theorem \ref{thm:non_linear_pricing_eqm}.] 
We start by examining  how the use of  concave pricing schemes may simplify FOP \eqref{eq:equilibrium-def}. Recall that both value functions and pricing functions are monotone non-decreasing and normalized to be $0$ at  $\bvec{0}$. For any concave buyer value function $u \in \C$, it is easy to see that the optimal pricing function $p$ simply equals $u$ (i.e., charging buyer exactly his imitative value) and ask the buyer to break ties in favor of the seller by picking $\bvec{x}^* = \arg\max_{\bvec{x} \in X} [u^*(\bvec{x}) - c(\bvec{x})]$ to maximize the seller's revenue. Consequently, the use of concave pricing simplifies FOP \ref{eq:equilibrium-def} to the following bi-level functional optimization problem: 
\begin{eqnarray}\nonumber 
  u^* = \argmax_{u  \in \C}  [  v(\bvec{x}^*) - p^*(\bvec{x}^* ) ],    
\text{ where }   \bvec{x}^* = \argmax_{\bvec{x} \in X} \big[ u^*(\bvec{x}) - c( \bvec{x} ) \big] 
\end{eqnarray} 

We fix a particular bundle $\bar{\bvec{x}}$ and  examine   what buyer value function $u \in \C$ would maximize the buyer's utility subject to that the trade will happen at bundle $\bar{\bvec{x}}$.  This results in the following \emph{functional optimization problem} (FOP) for the buyer with \emph{functional variable} $u$. 
\begin{lp}\label{lp:optimal_deception_concave_pricing}
	\maxi{ v(\bar{\bvec{x}}) - u(\bar{\bvec{x}}) }
	\st 
	\qcon{ u(\bar{\bvec{x}}) - c(\bar{\bvec{x}}) \geq u(\bvec{x}') - c(\bvec{x}') }{ \bvec{x}' \in X }
\end{lp}
where the constraint means the seller's optimal price  for  value function $u$ is $u(\bvec{\bar{x}})$ and thus the buyer best response amount is indeed $\bar{\bvec{x}}$.   The remaining proof relies primarily on the following lemma. 
%\begin{lemma}
	\begin{restatable}{lemma}{primelemmanonlinearpricing}
	\label{lemma:non_linear_pricing}
 The following concave function is optimal to FOP \eqref{lp:optimal_deception_concave_pricing}: 
  \begin{equation}\label{eq:opt-format-concave}
 \bar{u}(\bvec{x}) =\bar{p}  \cdot \min \{ \frac{x_1}{\bar{x}_1}, \cdots \frac{x_d}{\bar{x}_d}, 1\},  \quad \text{ where }  \bar{p} = \sup_{\alpha \in [0,1)} \frac{  c(\bar{\bvec{x}}) -c(\alpha \bar{\bvec{x}}) }{1 - \alpha}. 
 \end{equation}
\end{restatable}
%\end{lemma} 
Given this characterization, the buyer simply needs to look for the best $\bar{\bvec{x}}$. This then leads to the same characterization as in Theorem \eqref{thm:characterization} since Equation \eqref{eq:opt-format-concave} is the same as the value function characterized in Equation \eqref{eq:optimalformat_lem0}. The proof of  Lemma \ref{lemma:non_linear_pricing} is deferred to Appendix \ref{app_sec:proof-non-linear-pricing}.
\end{proof}
	
Theorem \ref{thm:non_linear_pricing_eqm} shows that more general class of pricing schemes may not help the seller to obtain more revenue. One might then wonder whether it at least never hurts since if that is the case, at least it would  never be a worse choice.  Unfortunately, 
our following example   shows that  a richer class of pricing schemes may   bring \emph{strict harm} to the seller and \emph{strict benefit} to the seller.  
% Therefore, according to Lemma \ref{lemma:non_linear_pricing} it is without loss of generality to assume the buyer's optimal imitative value function has the piece-wise linear  format \eqref{eq:optimalformat_concave_pricing}, and the concave pricing achieves the same utilities as linear pricing against this piece-wise linear value function. However, as shown in the following theorem, this does not hold for arbitrary sub-classes of concave pricing schemes.

\begin{example}[ The Risk of Overexploiting Buyer Incentives] \label{ex:hurt}
 There is a single type of divisible good to sell, i.e., $d=1$. Let the seller's production cost function be the convex function $c(x) = x^2$ and let the buyer's true value function $v(x)$ be the following piece-wise linear concave function  
\[
v(x) =
\begin{cases}
10x & 0 \leq x \leq 0.81 \\
8.1 & x > 0.81 
\end{cases}
\] 
\end{example}

Let $\P_C$ denote  the set of all  concave pricing schemes. The following proposition completes Example \ref{ex:hurt} and its proof can be found in Appendix \ref{app_sec:proof_concave_sub_class}. 
\begin{restatable}{proposition}{primepropsubclass}
%\begin{restatable}
	\label{thm:concave_sub_class}
For the instance   in Example \ref{ex:hurt},  there exists  pricing scheme class $\P $ with $\P_L \subset \P \subset \P_C$  such that when the seller changes from  linear pricing  class  $\P_L$ to the richer  class   $\P$, the seller's revenue strictly \emph{decreases} and the buyer's surplus strictly \emph{increases} at the equilibrium of \name{}.  
\end{restatable}

%\mh{proof here moved to appendix}
%\begin{proof}
%    We first analyze the situation of linear pricing. By the characterization in Theorem \ref{thm:characterization1}, we know that the optimal purchase bundle satisfies $x^* = \argmax_{\mathbf{x}\in X}[v(\mathbf{x}) - \mathbf{x} \cdot \nabla c(\mathbf{x})]$. Given $v(x)$ and $c(x)$ in Example \ref{ex:hurt}, this solves for $x^* = 0.81$ in the linear pricing setting. Furthermore, this gives $p^* = x^* \cdot \nabla c(x^*) = 1.3122$ and optimal imitative value function $u^* = 1.3122 \cdot \min\{x/0.81, 1\}$. The seller revenue in this case is $p^* - c(x^*) = 0.6561$.
%
%Next, we show that the seller's revenue will strictly decrease at equilibrium when using pricing class $\P = \P_L \cup \{ \tilde{p} \}$ that augments linear pricing class $\P_L$  with the following additional choice of a concave pricing function
%\[
%\tilde{p} (x) = \min(\sqrt{x}, \frac{5}{9}x + \frac{9}{20} - \epsilon)
%\]
%where  $\epsilon = 0.05$  is a   small constant. 
%
%    Consider the imitative value function $u^*(x) = \sqrt{x}$ and a particular linear pricing response $p > 0$. In this case, the buyer will purchase an amount $x' = \argmax_{x\in X}[u^*(x) - p\cdot x]$, implying $\frac{1}{2\sqrt{x}} = \frac{du^*(x')}{dx} = p$. Solving for $x'$ gives $x' = \frac{1}{4p^2}$. Now, we solve for the linear pricing response $p_L$ that maximizes the seller revenue.
%
%\begin{align*}
%    p_L &= \argmax_{p \in L}[p \cdot x' - c(x')] \\
%    &= \argmax_{p \in L}[p \cdot \frac{1}{4p^2} - \frac{1}{(4p^2)^2}] \\
%    &= \argmax_{p \in L}[\frac{1}{4p} - \frac{1}{16p^4}] \\
%    &= 1
%\end{align*}
%
%    Thus, the optimal linear pricing response to $u^*(x) = \sqrt{x}$ is $p_L = 1$. The buyer will purchase $x' = 0.25$, giving the seller a revenue of $1 \cdot 0.25 - 0.25^2 = 0.1875$. Finally, consider the pricing function $\tilde{p}(x)$ for the buyer's imitative value function $u^*(x) = \sqrt{x}$. We observe that $\frac{d}{dx}(\frac{5}{9}x + \frac{9}{20} - \epsilon) = \frac{5}{9} = \frac{1}{2\sqrt{0.81}} = \frac{d}{dx}(u^*(0.81))$, meaning $\argmax_{x \in X}[u^*(x) - p^*(x)] = 0.81$. Thus, the buyer can purchase $x = 0.81$ and the seller will get revenue $0.2439 - \epsilon = 0.1939$. This is strictly larger than the seller's revenue $0.1875$ from the optimal linear pricing scheme. Thus the seller's optimal pricing scheme from $\P$ is  $\tilde{p}(x)$. 
%
%    Finally, note that $\argmax_{x \in X}[v(x) - \tilde{p}(x)] = 0.81$, meaning the optimal bundle for the buyer to purchase when the seller responds with $\tilde{p}$ is $x = 0.81$. In this case the buyer surplus is $v(0.81) - \tilde{p}(0.81) = 8.1 - 0.9 + \epsilon > 8.1 - 1.3122 = v(0.81) - p_L \cdot 0.81$, meaning the optimal true buyer surplus given pricing function $\tilde{p}(x)$ is greater than the optimal true buyer surplus given any linear pricing response. Thus, $u^*(x)$ is an optimal imitative function under pricing class $\P$ and the seller revenue of $0.2439 - \epsilon = 0.1939$ is strictly lower than the seller revenue of $0.6561$ under linear pricing class $\P_L$.
%\end{proof}


==> backup - Copy/conclude.tex <==
%\section{Conclusions}
%This paper analyzes the equilibrium outcome of learning from \emph{strategically} revealed preferences. The equilibrium gives rise to a characterization on how a buyer will strategically respond to seller's learning algorithm and what the seller can expect to learn. Our work leaves many intriguing open questions: (1) What happens if the seller has some prior knowledge about buyer's value function? (2) What if the buyer does not perfectly know the seller's cost function? (3) What if the seller uses more sophisticated pricing schemes beyond linear pricing? Will it be easier or harder to game? 
%
%\todo{Expand this discussion, make it longer}
%% One implication of Theorem \ref{thm:imitation-opt} is that when learning from a strategic buyer, the seller is no better by learning through many rounds of interactions  than using the single-round preference-elicitation mechanism that simply asks the buyer to report his (possible untruthful) value function $u(\mathbf{x})$ and price against  $u(\mathbf{x})$. The main reason here is that the seller does not have any prior knowledge about the buyer's true value function $v(\mathbf{x})$. If some prior knowledge about $v(\mathbf{x})$ is available, then the seller's learning mechanism can leverage such prior knowledge to do better, and so do the classic mechanism design approaches. It is an intriguing open question to understand when the seller has prior knowledge, whether there is a separation between learning and classic mechanism design approaches. In particular, can learning do better than classic mechanism design when there is prior knowledge? 
%
%% Adjustments to our model based on real world settings offers a set of open questions. Similar to the question of increasing the seller's prior knowledge, what would be the optimal strategy if the buyer does not know the seller's cost function? What if buyer cares about utility throughout the learning phase? This is a more realistic characterization of the buyer and introduces a dependence on the seller's specific learning strategy. Additionally, pricing models other than linear could be considered. Another direction pertains to the seller response to buyer deception. Essentially, if the seller knows that the buyer is manipulative can the seller recover revenue by inferring back the true utility from the deceptive utility? This is a challenge for the current model as the seller does not actually learn the utility function and just learned a price. This could motivate a class of learning algorithms capable of learning a utility function rather than learning the optimal price.
%
%%
%%
%%\newpage
%%\section*{Broader Impact}
%%
%%With theoretical work, we do not have data biases or potential system failures, so the impact of these results are focused in offering a better understanding of the power and limitations of  machine learning algorithms for markets.  E-commerce systems such as online advertising platforms, online retailing platforms and crowdsourcing systems, can benefit from our principled analysis of basic market models. The analysis sheds light on how to design better pricing mechanisms that take into account buyers' strategic behaviors and balances agents' utilities. We believe no parties are put at disadvantages from this research. One goal is to help  to build a more organic economic system, which will benefit society in the long run.  
%
%
%% Behavior of a price learning strategy could be unpredictable when faced with an arbitrary buyer strategy so by classifying buyer responses according to the existence of a concave utility function, we offer sellers using price learning mechanisms the ability to detect non-imitative strategies. Consequently, a buyer should not be able to do better than the optimal imitative strategy while the seller cannot distinguish between honest buyer reporting and imitative deception. This offers a better understanding of market interactions between a single buyer and seller, but also shows buyer utility can be improved with deceptive practices.
%
\section{Conclusions}\label{sec:conclusion}

Motivated by optimal pricing against an unknown buyer, this paper put forwards a simple variant of the very basic pricing model by augmenting it with an additional stage of buyer commitment at the beginning. This motivation is driven by the seller's ignorance of the buyer's value function and thus have to price in the dark. We fully characterize the equilibrium of this new game model. The equilibrium reveals interesting insights about what the seller can learn, and how much seller revenue and   buyer surplus it may result in. We also show that more general class of pricing schemes may overfit the buyer's incentive and lead  to a pricing game that is even easier for the buyer to manipulate. 

%   the equilibrium outcome of learning from \emph{strategically} revealed preferences. The equilibrium gives rise to a characterization on how a buyer will strategically respond to seller's learning algorithm and what the seller can expect to learn. Our work leaves many intriguing open questions: (1) What happens if the seller has some prior knowledge about buyer's value function? (2) What if the buyer does not perfectly know the seller's cost function? (3) What if the seller uses more sophisticated pricing schemes beyond linear pricing? Will it be easier or harder to game? 

Our results opens the possibilities for many other interesting questions. For example, given the risk of using a too general class of pricing schemes, what class of pricing schemes is a good compromise between extracting revenue and  robust to buyer manipulations? Is linear pricing scheme the best such class or any other pricing scheme?  Second, as the first study of our setup, we have chosen to  focus  on a simple setup where the seller has completely no knowledge about the buyer's value function. An interesting question is, how the seller's learning and resultant revenue may increase when the seller has some prior knowledge about the buyer's values. In fact, one natural modeling question  is how to model the seller's prior knowledge about the buyer's  value function. Is the prior knowledge   about which subclass the value functions are from or  about what distribution the parameters of the value functions are from?  Finally, our model assumes that the buyer has full knowledge about the seller. An ambitious though extremely intriguing question to ask is what if the buyer also has incomplete knowledge about the seller and how to analyze the equilibrium under the information asymmetry from both sides. 

%  n this paper, we analyze the equilibrium outcome of learning to price from \emph{strategically} revealed preferences. We propose the model \name{} for this problem and provide succinct characterization of the equilibrium of this model. Our results show the optimal strategic deception for the buyer can without loss of generality be simply imitating some carefully designed piece-wise linear value function. We then instantiate this piece-wise linear value function with respect to specific seller types and show it's hard to compute this optimal imitative strategy in general. However, when the seller has \textit{convex} cost functions or only has single good to sell, we give explicit equilibrium results, including the specific optimal value function for the buyer to imitate and the final payoffs of both agents. Finally, we consider the \name{} under a richer class of pricing schemes used by the seller as a first step of counteracting the buyer's strategic manipulation. We tightly characterize the equilibrium of \name{} under this setting as well and show this additional power of pricing mechanisms doesn't necessarily improve the seller's revenue, which is similar to the spirit of over-fitting phenomenon in ML.

% We believe \name{} is a very natural model in which to learn the optimal price against an unknown strategic buyer, and that pursuing this line of work will be fruitful. Our work leaves many intriguing open questions: (1) What happens if the seller has some prior knowledge about buyer's value function? (2) What if the buyer does not perfectly know the seller's cost function? (3) What if the seller uses more sophisticated pricing schemes beyond the pricing schemes discussed in this paper? Will it be easier or harder to game? (4) What happens if the game happens between a single seller and multiple buyers? Does the competition help the seller to gain more revenue from the buyer?



% One implication of Theorem \ref{thm:imitation-opt} is that when learning from a strategic buyer, the seller is no better by learning through many rounds of interactions  than using the single-round preference-elicitation mechanism that simply asks the buyer to report his (possible untruthful) value function $u(\mathbf{x})$ and price against  $u(\mathbf{x})$. The main reason here is that the seller does not have any prior knowledge about the buyer's true value function $v(\mathbf{x})$. If some prior knowledge about $v(\mathbf{x})$ is available, then the seller's learning mechanism can leverage such prior knowledge to do better, and so do the classic mechanism design approaches. It is an intriguing open question to understand when the seller has prior knowledge, whether there is a separation between learning and classic mechanism design approaches. In particular, can learning do better than classic mechanism design when there is prior knowledge? 

% Adjustments to our model based on real world settings offers a set of open questions. Similar to the question of increasing the seller's prior knowledge, what would be the optimal strategy if the buyer does not know the seller's cost function? What if buyer cares about utility throughout the learning phase? This is a more realistic characterization of the buyer and introduces a dependence on the seller's specific learning strategy. Additionally, pricing models other than linear could be considered. Another direction pertains to the seller response to buyer deception. Essentially, if the seller knows that the buyer is manipulative can the seller recover revenue by inferring back the true utility from the deceptive utility? This is a challenge for the current model as the seller does not actually learn the utility function and just learned a price. This could motivate a class of learning algorithms capable of learning a utility function rather than learning the optimal price.

%
%
%\newpage
%\section*{Broader Impact}
%
%With theoretical work, we do not have data biases or potential system failures, so the impact of these results are focused in offering a better understanding of the power and limitations of  machine learning algorithms for markets.  E-commerce systems such as online advertising platforms, online retailing platforms and crowdsourcing systems, can benefit from our principled analysis of basic market models. The analysis sheds light on how to design better pricing mechanisms that take into account buyers' strategic behaviors and balances agents' utilities. We believe no parties are put at disadvantages from this research. One goal is to help  to build a more organic economic system, which will benefit society in the long run.  


% Behavior of a price learning strategy could be unpredictable when faced with an arbitrary buyer strategy so by classifying buyer responses according to the existence of a concave utility function, we offer sellers using price learning mechanisms the ability to detect non-imitative strategies. Consequently, a buyer should not be able to do better than the optimal imitative strategy while the seller cannot distinguish between honest buyer reporting and imitative deception. This offers a better understanding of market interactions between a single buyer and seller, but also shows buyer utility can be improved with deceptive practices.



==> backup - Copy/instantiate.tex <==
\section{Explicit Characterizations for Convex and Concave Costs}\label{sec:instantiation}
%\begin{proposition}\label{prop:hardness}
%For non-decreasing and concave cost function $c(\bvec{x})$, it is NP-hard to approximate the optimal seller revenue to be within ratio $1/d^{1 - \epsilon}$ for any $\epsilon > 0$, even when the buyer's value function is linear and known to the seller.   
%\end{proposition}

In this section, we instantiate Theorem \ref{thm:characterization} to both convex and concave cost functions, arguably the most widely adopted two classes of cost functions. In both cases, we give more explicit characterizations of the equilibrium outcome, including the buyer's optimal imitative value function as well as both agents' payoffs.  

%\subsection{ Convex Cost Functions} 


%\todo{For Minbiao: Can we somehow make this figure smaller but still clear, and also make captions look nicer. That "and" in left panel connects with right panel. }
%\mh{The smallest I can do, any size smaller than this is not so clear. Also, I was including pdf instead of img as figures, so the reader should be able to scale up the figure without loss of clearity to see the figure}

%\mh{Also, I am not sure what do you mean by tighter/smaller. If we want those two sub-figures closer/tighter, then the sub-caption's width will be smaller. Hence the whole length will be longer, which actually makes the whole figure larger because the length of the figure (i.e. \# lines occupied by the figure) increases as the two figures are closer. You can play with the parameter(i.e. change the percentage xx in \{xx/textwidth\}) in the latex code to see what I mean, I think the current version is the best I tried. }


% \noindent {\bf Instantiation I:  Explicit Characterizations for Convex Costs} 
Convex production costs are widely adopted in many applications   \cite{beato1985marginal,turvey1969marginal}.  When $c(\bvec{x})$ is convex and differentiable, we show the following explicit characterization about the equilibrium outcome. A graphical visualization for this theorem is depicted in the left panel of Figure \ref{fig:one-dimensional-characterization2}.

\begin{restatable}{restatethm}{primethmcharacterizationone}
%\begin{theorem}
	\label{thm:characterization1} When $c$ is convex and differentiable,  the piece-wise linear concave  value function $u^*(\bvec{x})$ defined by Equation \eqref{eq:optimal-format}, with $p^* = \bvec{x}^* \cdot \nabla  c(\bvec{x}^*)$ and $\bvec{x}^* = \arg \max_{\bvec{x} \in X} ~[v(\bvec{x}) - \bvec{x} \cdot \nabla  c(\bvec{x})]$, is an  optimal buyer imitative value function. 
%	the optimal buyer imitative  value function $u^*(\bvec{x})$  can w.l.o.g be specialized to the function $u^*(\bvec{x})$ from \eqref{eq:optimal-format} where . 

Under $u^*(\bvec{x})$, the trade  happens at bundle $\bvec{x}^*$ with payment $p^* = \bvec{x}^* \cdot \nabla  c(\bvec{x}^*)$.  The seller revenue $[\bvec{x}^* \cdot \nabla  c(\bvec{x}^*) - c(\bvec{x}^*)]$ is precisely the \emph{Bregman divergence} $D_{c}(\bvec{0},\bvec{x}^*)$ between $\bvec{0}$ and $\bvec{x}^*$. The buyer surplus is $[v(\bvec{x}^*) - \bvec{x}^* \cdot \nabla  c(\bvec{x}^*) ]$.
\end{restatable}
%\end{theorem}
%\mh{Some high-level intuition behind Theorem \ref{thm:characterization1}.}

\begin{figure}[!ht]
	\centering
	\begin{subfigure}{.49\textwidth}
		\centering 
		\includegraphics[page=1,width=.5\linewidth]{figures/convex-final2.pdf} 
		\caption{An example for convex cost: $v(x) = 64 \sqrt{x}$, $c(x) = x^2$. Theorem \ref{thm:characterization1} implies $x^* = 4$, $p^* = \nabla c(x^*) = 8$, seller utility $D_c(0,4) = 16$ \\and buyer utility $v(x^*) -  p^* \cdot  x^* = 96$.}
		\label{fig:sub1}
	\end{subfigure}
	\begin{subfigure}{.49\textwidth}
		\centering
		\includegraphics[page=1,width=.5\linewidth]{figures/concave-final2.pdf} 
		\caption{An example of one-dimensional concave costs: $v(x) = 4  x^{\frac{1}{4}}$, $c(x) = \sqrt{x}$. Theorem \ref{thm:characterization2} implies $x^* = 16$, $p^* = \frac{c(x^*)}{x^*}= 1/4$, seller utility is $0$ and buyer utility $v(x^*) -  p^* \cdot x^* = 4$.}
		\label{fig:sub2}
	\end{subfigure}
	\caption{Illustration of the equilibrium characterization:  $v(x)$ is buyer's true value function, $c(x)$ is  the seller's cost function, and $u^*(x)$ is the  optimal buyer imitative value function. 
		%		 and the payment function will be $p\cdot x$ where $p\geq0$. If $\exists x >0$ such that $p \cdot x < c(x)$, the buyer will choose that amount $x$ for him for earn positive utility which results in a negative utility for the seller. Therefore, the seller will set the price $p$ such that the payment function $p\cdot x \geq c(x)$, $\forall x>0$ \big( i.e. $p=\infty$ if $c(x)$ is convex and $p=\nabla c(0)$ if $c(x)$ is concave\big) which means the buyer can only buy 0 amount.
\vspace{-2mm}	
} 
	\label{fig:one-dimensional-characterization2}
\end{figure}

We now consider  concave costs and prove the following characterization. A graphical visualization for the theorem is depicted in the right panel of Figure \ref{fig:one-dimensional-characterization2}. 

\begin{restatable}{restatethm}{primethmcharacterizationtwo}
%\begin{theorem}
	\label{thm:characterization2} When  $c(\bvec{x})$ is     concave, the piece-wise linear concave  value function $u^*(\bvec{x})$ defined by Equation \eqref{eq:optimal-format}, with $p^* =  c(\bvec{x}^*)$  and $\bvec{x}^* =\arg \max_{\bvec{x} \in X} ~[v(\bvec{x}) - c(\bvec{x})]$, is an  optimal buyer imitative value function.  

Under $u^*(\bvec{x})$, the trade  happens at bundle $\bvec{x}^*$ with payment $p^* =  c(\bvec{x}^*)$.  The seller revenue will be $0$. The buyer extracts the maximum possible surplus   $ \max_{\bvec{x} \in X} [v(\bvec{x}) -    c(\bvec{x}) ]$. 
\end{restatable}
%\end{theorem}

\vspace{-2mm}
Graphical visualizations for the above two theorems are depicted in Figure \ref{fig:one-dimensional-characterization2}.  Note that both examples in Figure \ref{fig:one-dimensional-characterization2} show the sub-optimality of imitating $u^*(x) = c(x)$ for the buyer. To see this, note  $u^*(x) = c(x)$ makes the game zero-sum. To guarantee non-negative revenue, the seller must pick a price $p$ such that the line $p\cdot x$ is always above $u^*(x)$. A buyer imitating $u^*(x) = c(x)$ will end up purchasing a $0$ amount in both cases, and thus are sub-optimal for him.     

 
An important conceptual message from Theorem \ref{thm:characterization2} is that when the seller production cost is concave and known to the buyer, the buyer can always come up with  an imitative value function which squeeze the seller's revenue to its extreme, i.e., $0$.\footnote{In real practice, the buyer can slightly deviate from his value function to given a small  $\epsilon$ amount of incentive for the seller to strictly prefer production.}  Under the seller's optimal imitative value function, the trade will happen at his most favorable bundle amount $\bvec{x}^*$ and  the seller pays just the cost function $c(\bvec{x}^*)$ to the seller.  

Theorem \ref{thm:characterization2}  is certainly bad news for the seller.  However, it is a \emph{descriptive}  result and only shows it is possible for the buyer to achieve maximum possible surplus.  Our next result brings somewhat good news to the seller. Specifically, we show it is NP-hard for the buyer to optimize, even approximately,  his optimal surplus. The hardness holds even when the production cost function $c(\bvec{x})$ is concave, in which case the surplus is characterized by Theorem \ref{thm:characterization2}. This shows that even though in theory the buyer can derive large surplus from strategic manipulation, even approximately figuring out such an optimal manipulation is  impossible in general, unless P = NP.

\begin{restatable}{restatethm}{primethmhardness}
%\begin{theorem}
	\label{prop:hardness}[Intractability of Equilibrium] 
	% 	Define the ``fixed-$\bvec{p}$ OP \eqref{lp:buyer-simple-thm}" problem  as solving OP \eqref{lp:buyer-simple-thm}  over only variable $\bvec{x}$ but with a given price vector $\bvec{p}$.   It is NP-hard to approximate the fixed-$\bvec{p}$ OP \eqref{lp:buyer-simple-thm} to be within ratio $1/d^{1- \epsilon}$ for any $\epsilon >0$, even when   the production cost function $c(\bvec{x})$ is concave. 
	It is NP-hard  to approximate the buyer equilibrium  surplus in \name{}  games to be within ratio $1/d^{1- \epsilon}$ for any $\epsilon >0$. This hardness result holds  even when    the production cost function $c(\bvec{x})$ is concave and  the buyer's true value function $v(\bvec{x}) $ is simply the linear function $ \sum_{i=1}^d x_i$.  
\end{restatable}
%\end{theorem}

Formal proofs for both equilibrium characterizations and the hardness of approximating the buyer equilibrium surplus can be found in Appendix \ref{app_sec:proof-section-initantiation}. We note that an intriguing open question is whether optimal imitative value function can be computed for \emph{convex} production cost $c(\bvec{x})$.  In this case, the optimal bundle $\bvec{x}^* $ can be explicitly expressed as $\bvec{x}^* = \argmax_{\bvec{x}} [ u(\bvec{x}) - \bvec{x} \cdot \nabla c(\bvec{x})]$  for any value function $u$, however how to derive the optimal $u^*$ remains challenging.   

==> backup - Copy/intro.tex <==
\section{Introduction}
Pricing  is a basic question in microeconomics \cite{mas1995microeconomic} as well as a ubiquitous problem in today's digital markets \cite{den2015dynamic}.  In its textbook style setup, there are two agents: a  buyer (he)  and a seller (she). The seller produces $d$ types of \textit{divisible} goods for sale and has production cost $c(\bvec{x})$ for producing  \emph{bundle} $\bvec{x} \in \RR_+^d$ of the $d$ goods.  Using a standard linear pricing scheme with unit price  $p_i$ for goods $i\in[d]$, the seller charges the  buyer   $\bvec{x} \cdot \bvec{p}$ when he purchases bundle $\bvec{x} \in \RR_+^d$ under price vector $\bvec{p} \in \RR_+^d$.  Naturally,  the buyer's optimal bundle for purchase   depends on his \emph{value} function $v(\bvec{x})$ about the products. We assume that, given price vector $\bvec{p}$,   the rational buyer will always  pick the optimal bundle that maximizes his quasilinear utility $[v(\bvec{x}) - \bvec{x} \cdot \bvec{p}]$.  The key question of interest is how the seller can compute   the revenue-maximizing optimal prices assuming rational   buyer purchase behaviors.  %  with the knowledge of the buyer's value function $v(\bvec{x})$. 


%  Specifically, a buyer who looks to buy \emph{fractional} bundles of $d$ goods repeatedly interacts with a seller. At each round of interaction, the seller posts a price $\bvec{p}\in \RR_+^d$ and the buyer responds with buying bundle $\bvec{x}\in \RR_+^d$ that can maximize his utility $v(\bvec{x}) - \bvec{x} \cdot \bvec{p}$ where $v$ is his valuation function over the goods. The seller receives the revenue $\bvec{x} \cdot \bvec{p} - c(\bvec{x})$ after the buyer purchases $\bvec{x}$ where $c$ is her cost function of producing the goods. The seller's revenue maximization problem is then to set prices that can maximize her revenue against the buyer.

The above basic problem can be easily solved if the seller has access to the buyer's value function $v(\bvec{x})$. However, in practice,  this value function is usually private  and unknown to the seller. To address this challenge, there has been a rich line of recent research which looks to design the optimal pricing scheme against an unknown buyer. Some of these work  have adopted  learning-based approaches that aim to compute the profit maximizing price by interacting with the buyer and gleaning information about the buyer's utility function \cite{amin2015online,roth2016watch,roth2020multidimensional}.  These are motivated by the wide spread of e-commerce today where the seller can repeatedly interact with the same buyer or buyers from the same population with similar preferences. For example,  in \emph{online advertising},  ad exchange platforms learn to price advertisers from past behaviors; in \emph{online retailing},   retailers learn to price customers from their past purchase history;  and in \emph{crowdsourcing},  platforms learn to reward workers' efforts.  Another line of works look to design dynamic pricing mechanisms that dynamically adjusts the price based on the observed past buyer purchase behaviors with the objective of maximizing the aggregated total revenue   \cite{amin2013learning,amin2014repeated,mohri2014optimal,mohri2015revenue,vanunts2019optimal}. 

A key challenge of pricing against such unknown buyers, regardless through learning or dynamic pricing, is that the  buyer may manipulate his responses  in order to mislead the seller's algorithm and induce more favorable outcomes for themselves. This is a fundamental issue when learning from strategic data sources, and is particularly relevant in this pricing setup due to the  strategic nature of the problem.   In this case,  the buyer controls the information content to the seller,  therefore he naturally has incentives to utilize this advantage to gain more payoff by strategically misleading the seller's   algorithms.  Indeed, as observed in previous studies,  online advertisers may strategically respond to an ad exchange platform's prices in order to induce a lower future price \cite{korula2015optimizing}; Consumers strategically time their purchases in order to obtain lower prices at online retailing platforms  \cite{li2014consumers}.  

To understand the limits of the seller's optimal pricing against such a strategic and possibly manipulative buyer, we put forward a natural model which   augments the above basic pricing problem with only one additional step --- i.e.,  we assume that the game starts with the buyer  \emph{committing} to a different value functions, coined the \emph{imitative value function}, after which the seller will compute the optimal pricing scheme against this imitative buyer value function.  The buyer's commitment to an imitative value function captures a simple yet powerful buyer manipulation strategy that can be used against any seller learning algorithms ---  that is, the buyer simply  behaves consistently according to this  imitative value function during the entire interaction process. Intuitively, the motivation of such commitment assumption comes directly from the fact that the seller has no information about the buyer and  has to optimize pricing ``in the dark''. Consequently, if the buyer consistently behaves according to some different imitative value function, the seller is not able to distinguish this buyer from another buyer who truly has the value function (see more justifications of the commitment assumption in Section \ref{sec:model}). Moreover, such an imitation strategy is also easy to execute in practice by the buyer regardless whether the seller is learning from him or is adopting dynamic pricing schemes. In fact, the buyer could   even just  report his imitative value function to the buyer directly at the beginning of any interaction. In this situation, no learning or dynamic pricing will be needed as the buyer will indeed always behave according to the imitative value function. Therefore,  all the seller can do is  to directly apply the optimal pricing scheme for the buyer's imitative  value function.  

We remark that such imitation-based manipulation strategy has attracted much interest in   recent works, with similar motivations as us --- i.e., trying to understand how to manipulate learning algorithm or conversely, how to design strategy-aware learning algorithms to mitigate such manipulation.  However, most of these works have focused on the general Stackelberg game model \cite{gan2019imitative,birmpas2020optimally} as well as the Stackelberg security games \cite{gan2019manipulating,nguyen2019imitative,nguyen2020decoding}. Our optimal pricing problem is also a Stackelberg model and thus a natural fit for the study. The crucial difference between our work and previous studies is that both agents in our model have \emph{continuous} utility functions whereas all these previous works \cite{gan2019imitative,gan2019manipulating,nguyen2019imitative,birmpas2020optimally}  have discrete agent utility functions. Therefore, our model leads to a \emph{functional} analysis and optimization problem, which is more involved. Fortunately, we show that the optimal functional solution can still be characterized by leveraging the structure of the pricing problem. 

%  Recent works have also started to examine how the follower may  strategically mislead the leader's learning algorithms \cite{gan2019imitative,gan2019manipulating,nguyen2019imitative,birmpas2020optimally}.   They examined certain payoff imitation strategies as well but whether such an imitative strategy is optimal in general are unclear.  Moreover, the structural difference of these games from pricing games makes these results incomparable to ours. For example, \cite{gan2019manipulating,nguyen2019imitative} prove that in security games it is best for the attacker to imitative a zero-sum game payoff whereas in pricing problem we argue that this is sub-optimal. There have also works studying how to strategically respond to a particular class of learning algorithms, specifically no-regret algorithms, in general bi-matrix games \cite{deng2019strategizing} or in auctions \cite{braverman2018selling}. However, in our model, the seller is allowed to use any effective learning algorithm.   



% There is also a body of related work on learning the buyer's value function directly. In this line of work, their goal is to learn and predict the buyer's behavior instead of optimizing seller prices. Classic economic research  studies when it is possible to find a buyer utility function $u(\bvec{x})$ that explains the observed data $\{ (\bvec{p}_t, \bvec{x}_t )\}_{t=1}^T$ after the seller interacts with the buyer for $T$ rounds, assuming a utility-maximizing buyer. Specifically, the goal is to guarantees $\bvec{x}_t$ maximizes $u(\bvec{x})$ subject to $\bvec{p}_t \cdot \bvec{x} \leq \bvec{p}_t \cdot \bvec{x}_t$ for any $t \in [T]$. This is sometimes also called \emph{rationalizing the data}. Since \cite{samuelson1938note}, there has been a rich line of economic research on this problem termed as \textit{learning from revealed preferences}. We refer the reader to an excellent survey by Varian \cite{varian2006revealed}.

%How does  revealed preference theory relate to computer science, and particularly, machine learning?   The study of revealed preferences is intrinsically a function fitting problem. However, different from standard function fitting for (variable, value) sequences, here we look for a function $u(\bvec{x})$ to \emph{fit the buyer's revealed preferences}, i.e.,  to guarantee that the buyer's best bundle to price $\bvec{p}_t$ is $\bvec{x}_t$ for any $t$. Nevertheless, one can ask similar  and equally important machine learning questions such as how many data points are needed to learn a good predictor for buyer responses or  how many data points are needed to learn the underlying utility function  $u(\bvec{x})$ \cite{beigman2006learning,zadimoghaddam2012efficiently,balcan2014learning}. Going beyond the fitting/prediction of buyer behaviors, recent works leverage advances in ML algorithms and study how to directly learn the optimal price  from the buyer's revealed preferences \cite{amin2015online,roth2016watch,roth2020multidimensional} (note that a seller may be able to learn the optimal price without learning the buyer's utility function). These are motivated by the wide spread of e-commerce today including in \emph{online advertising}  (where ad exchange platforms learn to price advertisers from past behaviors), \emph{online retailing} (where retailers learn to price customers from their past purchase history), and \emph{crowdsourcing} (where platforms learn to reward workers' efforts). 

%Despite significant recent progress, all works on pricing against an unknown buyer so far have relied on a crucial assumption. That is, the buyer must honestly interact with the seller. Under this assumption,  recent works developed efficient algorithms to learn  the revenue-optimal \cite{amin2015online,roth2016watch} or welfare-optimal prices \cite{roth2020multidimensional}  in natural setups.  Motivated by these concerns, the presented work seeks to understand price learning from such a strategic buyer.  We aim to answer the following research questions: 
%
%\vspace{-1mm}
%\begin{quote}
%	\it  When learning prices from an unknown buyer, how will the buyer strategically respond to the seller's learning algorithm?  What can the seller expect to learn? And how will such strategically revealed responses affect both agents' objectives?   
%\end{quote}
%\vspace{-1mm}
%
%
%\hf{okay, so now you described the problem to study, what is the model you are proposing? Should describe the model here.}
%
%We consider a seller who looks to learn the optimal price against an unknown buyer. The seller produces $d$ divisible goods with a publicly known production cost function $c(\bvec{x})$. She uses linear pricing  scheme parameterized by a price vector $\bvec{p} \in \RR_+^d$, and thus charges $\bvec{p} \cdot \bvec{x}$ for $\bvec{x}$ bundle of goods.  The buyer has a  \emph{private}  value function $v(\bvec{x})$. We consider the scenario that the seller aims to compute an optimal price which can maximize her revenue against this unknown buyer. On the other hand, if the buyer controls the flow of information to the seller, how should he utilize this advantage to gain more payoff through revealing information which is good for him. 

% They interact for $T$ rounds and generate trading data $(\bvec{p}_1, \bvec{x}_1), \cdots, (\bvec{p}_T, \bvec{x}_T)$. The seller looks to design a price learning algorithm that maps any past  data $(\bvec{p}_1, \bvec{x}_1), \cdots, (\bvec{p}_{t-1}, \bvec{x}_{t-1})$ to a new price $\bvec{p}_t$, with the objective of outputting an optimal price at round $T$ for some carefully chosen $T$.  We note that this is the textbook setup for revealed preferences  (e.g., divisible goods, linear pricing, single buyer  \cite{mas1995microeconomic,rubinstein2012lecture}).  These modelling choices all  have variants or generalizations, but the description here is arguably the most basic. Previous  studies of learning algorithms \cite{amin2015online,roth2016watch,roth2020multidimensional}  assumed that the buyer's response at each round is always an honest best response according to a quasi-linear buyer utility function, i.e., $\bvec{x}_t = \argmax_{\bvec{x}} [v(\bvec{x}) - \bvec{p}_t \cdot \bvec{x}]$ for any $t$. The only difference of our model from previous studies is that we allow the buyer to \emph{strategically} and \emph{adaptively} pick his response sequence $\bvec{x}_1, \cdots,, \bvec{x}_{T}$,  with the objective of tricking the seller's learning algorithm to induce a favorable  final price $\bvec{p}_T$ for himself. That said, both agents care about only the final learning outcome $\bvec{p}_T$. This is often assumed in models of learning from revealed preferences  and is consistent with previous works \cite{amin2015online,roth2016watch,roth2020multidimensional} (see more discussions in Section \ref{sec:model}).

\subsection{Our Results and Implications}\label{sec:results}
Given the effectiveness  and easy applicability  of the buyer's imitative strategy described above, this paper studies what the optimal buyer imitative value function is and how it would affect buyer's surplus and the seller's revenue.  Our main result provides a full characterization  about the optimal buyer imitative value function.  We show that the optimal buyer imitative value function $u^*$ features a specific  bundle of products $\bvec{x}^*$ that is most desirable to the buyer. Interestingly, it turns out that   $u^*$ is a Leontief-type  piece-wise linear concave value function \cite{allen1967macro}   such that the buyer would only  proportionally value a fraction of the desired bundle   $\bvec{x}^*$ and nothing else. %Through such a value function, the buyer will be able to successfully induce the selling price such that under that price his optimal  bundle, under imitative value function $u^*$, is precisely  $\bvec{x}^*$. 
Moreover, we also characterize the  seller revenue and buyer surplus at equilibrium as well as necessary and sufficient conditions under which the seller obtains strictly positive revenue. 


The optimal buyer imitative value function turns out to depend crucially on the seller's production cost function. When the cost function is concave, we show that the optimal buyer imitative value function $u^*$  will ``squeeze'' the  seller revenue essentially to $0$. The fortunate news for the seller, however, is that finding out the $u^*$ turns out to be an NP-hard task for the buyer. In fact, we prove that it is NP-hard to find the $u^*$ that can guarantee a polynomial faction of the optimal buyer surplus. %This intractability result conveys  positive news to the seller.  
For the   widely  adopted \emph{convex}  production cost, we show that the equilibrium seller revenue is  the Bregman divergence  between production $\bvec{0}$ and the $\bvec{x}^*$ bundle mentioned above. This illustrates an interesting message that convex production  costs are ``better'' at  handling buyer's strategic manipulations. Note that production costs are indeed more often believed to be convex since  economic models typically assume that marginal costs increase as quantity goes up \cite{shephard1974law,samuelson1998microeconomics}. 
% \mh{Concave costs is referred as diminishing marginal cost in economics. Economies of scale show that a company can usually decrease their cost per unit of production when they produce goods in mass quantities. However, as the production quantities get higher and higher until reaching the efficient volume, marginal cost will eventually rise again which results in a convex cost function. But, in general, economic models assume that marginal costs increase as quantity goes up.}

All our characterizations so far focus on the standard \emph{linear} pricing scheme. Our last result examines the possibility of using a more general class of pricing  schemes  to address the buyer's strategic manipulation. Surprisingly, we show that for the strictly more general class of concave pricing functions (i.e., the seller is allowed to use any concave function as a pricing function), the equilibrium will remain the same as described above. Therefore, the more general pricing schemes do not necessarily help to address buyer's manipulation behavior.  In fact, we show that there exist  examples where strictly \emph{broader} class of pricing functions leads to strictly worse seller revenue. This is because more general pricing schemes may ``overfit'' buyer's incentives, which renders it easier to manipulate. This illustrates an interesting phenomenon in learning from strategic data sources and shares similar spirit to  \emph{overfitting}  in standard machine learning tasks.  

\vspace{-0.03em}
% Different from previous works which designs efficient algorithms to learn the optimal price, our goal here is to characterize how the buyer will \emph{strategically}  respond to a learning algorithm and what the seller can learn from such responses.  We first show that  the optimal buyer response to any effective seller learning algorithm can without loss of generality be simply  imitating some carefully chosen concave value function $u^*(\bvec{x})$, i.e., responding with $\bvec{x} = \argmax_{\bvec{x}} [u^*(\bvec{x}) - \bvec{p} \cdot \bvec{x}]$ for any $\bvec{p}$.   \hf{why still revealed preferences thing here? }

%Leveraging the above characterization, we are then able to characterize the optimal $u^*$  as well as the learning outcomes. We show that $u^*$ can always be an additive  concave function that is a truncation of a linear function, with  parameters  computed from an optimization program depending on $c(\bvec{x})$ and $v(\bvec{x})$. Unfortunately, we prove that it is NP-hard to approximate this optimization program within any polynomial factor, even for  \emph{concave} $c(\bvec{x})$. However, when the seller's cost function $c(x)$ is \textit{concave}, our result shows that even though figuring out an optimal manipulation is impossible for the buyer, we prove that in theory the buyer can derive extreme large surplus from strategic manipulation and squeeze the seller's revenue to be zero. On the other hand, for \emph{convex} cost function $c(\bvec{x})$  as widely adopted in economics \cite{beato1985marginal,turvey1969marginal},   we are able to give more explicit characterization of $u^*$ which allows us to show that the ultimately learned price vector will be the marginal production cost $\nabla c(\bvec{x}^*)$ at certain bundle $\bvec{x}^*$ and the seller's revenue is simply the Bregman divergence  between production $\bvec{0}$ and $\bvec{x}^*$. Interestingly, the optimal $u^*$  here cannot simply be the $c(x)$ as one might first think of.   \hf{this is not updated...our results are different now. }

 %As another case study,  for one-dimensional (i.e., a single product) concave $c(x)$, the optimal $u^*$ can be explicitly characterized as well. In this case, the seller will learn a price that gives her $0$ revenue. The buyer will achieve the maximum possible utility, i.e., $\max_{x} [v(x) - c(x)]$, using strategic responses. Interestingly, the optimal $u^*$  here cannot simply be the $c(x)$ as one might first think of.  \hf{this is not updated...our results are different now. }

% Finally, we take one step further to explore what can the seller do to counteract the buyer's strategic deception. We enable the seller to use a richer class of pricing schemes instead of pricing schemes only. Interestingly, it turns out that this additional power does not necessarily help the seller to gain more revenue but may hurt the seller, which shares a same spirit as over-fitting in machine learning literature (see more details in Section \ref{sec:concave}).

\subsection{Additional Related Works}\label{sec:related}
Due to space limit, here we only briefly discuss the most related works while refer readers to Appendix \ref{append:sec:related} for more detailed discussions and comparisons. Closely related to ours is a recent study by  Tang and Zeng \cite{tang2018price}. They study  the bidders' problem of committing to ``imitate'' a fake value \emph{distribution} in auctions and acting consistently as if the  bidder's  value were from the fake  distribution. This is similar in spirit to our buyer's commitment to an imitative value \emph{function}. However, there is significant difference betweens  our setting and  that of \cite{tang2018price}, which leads to very different conclusions as well. Specifically, the seller in \cite{tang2018price} auctions a single indivisible item with no production costs whereas our seller sells multiple divisible items with production costs.   Another recent work \cite{nedelec2020robust} also  studies buyer's strategic manipulation  against seller's pricing algorithms, but in a single-item multi-buyer situation. Moreover, they assume a fixed  seller  learning strategy (thus not adaptive to buyer's strategy) with separated  exploration-exploitation phases motivated by \cite{amin2013learning}. 
%This is an important difference because with $0$ production cost, the optimal manipulation in our case is trivial,  i.e. the buyer will imitate a value function of 0.  However, this trivial solution does not arise in the model of \cite{tang2018price} because in their setup there are multiple buyers (bidders) and the competition among bidders increases the auctioneer's revenue despite bidders' imitative or faking behaviors. This is the second key difference between our work and \cite{tang2018price}. Therefore,  our work illustrates  how the production cost can affect the buyer's strategic manipulation and the seller's revenue whereas the work of Tang and Zeng \cite{tang2018price}  sheds light on how the bidders' competition affect the auctioneer's mechanism design and ultimate revenue. Though these two aspects are not comparable,  we  believe they are both interesting for a deep understanding. 
Another  very relevant literature is  learning the optimal prices or optimizing aggregated total revenue by repeatedly  interacting with a single buyer   \cite{amin2013learning,amin2014repeated,mohri2014optimal,mohri2015revenue,vanunts2019optimal}.  These   works all focus on designing learning algorithms that can learn from strategically  buyer responses. Our work  complements  this literature by studying the limits of what learning algorithms can achieve.  Moreover, the setups of these previous works are also different from us -- they either assume buyer values are drawn from distributions  \cite{amin2013learning,amin2014repeated,mohri2015revenue}  or the seller sells a single indivisible good  with discrete agent utilities. Thus, their results are not comparable to us.


There have also been studies on learning the optimal prices from \emph{truthful} revealed preferences, i.e., assuming the buyer will honestly best respond to seller prices \cite{beigman2006learning,zadimoghaddam2012efficiently,balcan2014learning,pmlr-v119-zhang20f,amin2015online,roth2016watch,roth2020multidimensional}. Our works try to understand if the assumption of truthful revealed preferences does not hold and if the buyer will strategically respond to the seller's learning, what learning outcome could be expected when the buyer simply imitates a different value function that is  optimally chosen. From this perspective, these works serve as a key motivation for the present paper.   More generally, our work subscribes to the general line of research on learning from strategic data sources. 
Most works in this space has focused on classification  \cite{bruckner2011stackelberg,hardt2016stratclass,zhangincentive,dong:ec18,milli:fat19,hu:fat19,chen2020learning},  regression problems \cite{Perote2004StrategyproofEF,dekel2010incentive,chen:ec18} and distinguishing distributions \cite{zhang2019distinguishing,zhang2019samples}. Our work however focuses on learning the optimal pricing scheme.  

        


 


% There have also works studying how to strategically respond to a particular class of learning algorithms, specifically no-regret algorithms, in general bi-matrix games \cite{deng2019strategizing} or in auctions \cite{braverman2018selling}. However, in our model, the seller is allowed to use any effective learning algorithm.    


%The seller is still willing to produce the product even if the price is 0 because it costs her nothing to produce. Secondly, as we just mentioned, we consider the setup with multiple items for sell while a significant part of the literature only considers single-item auctions \cite{amin2013learning,amin2014repeated,mohri2014optimal,mohri2015revenue,vanunts2019optimal,tang2018price}. 


%The study of strategic buyer behaviors in pricing problems are natural and rich. The literature of dynamic pricing studies how to design  mechanisms to achieve the optimal revenue when repeatedly interacting with strategic buyers. One line of this literature assumes the buyer at each round is a fresh new and myopic buyer \cite{kleinberg2003value,babaioff2015dynamic,besbes2009dynamic,broder2012dynamic,den2014simultaneously,keskin2014dynamic,wang2014close}. More similar to us is the second line of this literature, which assumes that the seller interacts with a single buyer repeatedly \cite{amin2013learning,amin2014repeated,mohri2014optimal,mohri2015revenue,vanunts2019optimal}.  Similar to us,  they also consider the buyer's strategic behavior  that potentially tricks the seller's learning algorithm.  Some of these models \cite{amin2013learning,amin2014repeated,mohri2015revenue}  assume that the buyer's values for goods  are drawn from  distributions (a.k.a., demand distribution) and consequently his best responses to seller prices are  random with randomness inherited from his value distribution. However,  our model originates from the revealed preference literature which assumes that  the buyer has a  unknown but fixed value function that drives his  purchase responses.  Such a response is the solution to buyer's optimization problem while not from a random distribution.  However,  it similarly requires learning because the seller does not know the buyer's value function.  There have also been models that  consider unknown but fixed buyer values \cite{mohri2014optimal,vanunts2019optimal}. However, their works   still significantly differ from   ours. First, our model has multiple divisible goods to sell whereas the mentioned works above have a single indivisible good. Selling multiple divisible goods is fundamentally different from, and much more challenging than, selling a single indivisible goods. In the former case, the buyer's value is a \emph{multi-dimensional function} whereas in the later the buyer's value is a single real number.   Second, due to such significant difficulty, we focused on a less ambitious goal of characterizing what the seller can learn using an “effective” learning algorithm whereas other mentioned works directly design good/optimal pricing algorithms.  

 


==> backup - Copy/macros.tex <==
\newtheorem{theorem}{Theorem} 
\newtheorem{restatethm}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{example}{Example}
%\newtheorem{thm}[theorem]{Theorem}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{note}[theorem]{Note}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{conjecture*}{Conjecture}
\newtheoremstyle{nonindented}{1ex}{1ex}{}{}{\bfseries}{.}{.5em}{}
\newtheoremstyle{indented}{1ex}{1ex}{\itshape\addtolength{\leftskip}{0.6cm}\addtolength{\rightskip}{0.6cm}}{}{\bfseries}{.}{.5em}{}
\theoremstyle{nonindented}
%\newtheorem{domain}{Game Domain}
\theoremstyle{indented}
%\newtheorem{question}{Question}[section]
%\newtheorem*{direction*}{Research Direction}
%\newtheorem*{conjecture*}{Conjecture}
\theoremstyle{plain}



\newenvironment{proofof}[1]{\begin{proof}[Proof of #1]}{\end{proof}}
\newenvironment{proofsketch}{\begin{proof}[Proof Sketch]}{\end{proof}}
\newenvironment{proofsketchof}[1]{\begin{proof}[Proof Sketch of #1]}{\end{proof}}

\newenvironment{alg}{\begin{algorithm}\begin{onehalfspace}\begin{algorithmic}[1]}{\end{algorithmic}\end{onehalfspace}\end{algorithm}} 

\newcommand{\mult}{\times}
\newcommand{\cross}{\times}
\newcommand{\by}{\times}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bvec}[1]{\boldsymbol{ #1 }}
\newcommand{\card}[1]{\left| #1 \right|}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}
\newcommand{\bigunion}{\bigcup}
\newcommand{\bigintersect}{\bigcap}
\newcommand{\sm}{\setminus}
\newcommand{\floor}[1]{\lfloor {#1} \rfloor}
\newcommand{\ceil}[1]{\lceil {#1} \rceil}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}
\newcommand{\iid}{i.i.d.\ }

\newcommand{\lt}{\left}
\newcommand{\rt}{\right}


\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}

%Operators: These operators are such that a subscript appears below
%in \[ \] math mode, and to the bottom right in regular $ $ math mode

%regular version
\def\pr{\qopname\relax n{Pr}}
\def\ex{\qopname\relax n{E}}
\def\min{\qopname\relax n{min}}
\def\max{\qopname\relax n{max}}
\def\argmin{\qopname\relax n{argmin}}
\def\argmax{\qopname\relax n{argmax}}
\def\avg{\qopname\relax n{avg}}


%bold version
\def\Pr{\qopname\relax n{\mathbf{Pr}}}
\def\Ex{\qopname\relax n{\mathbf{E}}}
\def\supp{\qopname\relax n{\mathbf{supp}}}
\def\Min{\qopname\relax n{\mathbf{min}}}
\def\Max{\qopname\relax n{\mathbf{max}}}
\def\Argmin{\qopname\relax n{\mathbf{argmin}}}
\def\Argmax{\qopname\relax n{\mathbf{argmax}}}
\def\Avg{\qopname\relax n{\mathbf{avg}}}
\def\vol{\qopname\relax n{\mathbf{vol}}}
\def\aff{\qopname\relax n{\mathbf{aff}}}
\def\conv{\qopname\relax n{\mathbf{convexhull}}}
\def\hull{\qopname\relax n{\mathbf{hull}}}

\newcommand{\expect}[2][]{\ex_{#1} [#2]}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\RRp}{\RR_+}
\newcommand{\RRpp}{\RR_{++}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}

\def\A{\mathcal{A}}
\def\B{\mathcal{B}}
\def\C{\mathcal{C}}
\def\D{\mathcal{D}}
\def\E{\mathcal{E}}
\def\F{\mathcal{F}}
\def\G{\mathcal{G}}
\def\H{\mathcal{H}}
\def\I{\mathcal{I}}
\def\J{\mathcal{J}}
\def\K{\mathcal{K}}
\def\L{\mathcal{L}}
\def\M{\mathcal{M}}
\def\P{\mathcal{P}}
\def\R{\mathcal{R}}
\def\S{\mathcal{S}}
\def\O{\mathcal{O}}
\def\T{\mathcal{T}}
\def\V{\mathcal{V}}
\def\U{\mathcal{U}}
\def\X{\mathcal{X}}
\def\Y{\mathcal{Y}}

\def\eps{\epsilon}
\def\sse{\subseteq}

\def\SS{\mathbb{S}}

\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\Bmat}[1]{\begin{Bmatrix} #1 \end{Bmatrix}}
\newcommand{\vmat}[1]{\begin{vmatrix} #1 \end{vmatrix}}
\newcommand{\Vmat}[1]{\begin{Vmatrix} #1 \end{Vmatrix}}
\newcommand{\mat}[1]{\pmat{#1}}
\newcommand{\grad}{\bigtriangledown}
\newcommand{\one}{{\bf 1}}
\newcommand{\zero}{{\bf 0}}


\newcommand{\eat}[1]{}


\newcommand{\hl}[1]{{\bf \color{red}#1}}
\newcommand{\todo}[1]{{\hl{To do: #1}}}
\newcommand{\change}[1]{{\hl{#1}}}
\newcommand{\todof}[1]{{\hl{ (Todo\footnote{\hl{\bf  To do: #1}})}}  }
\newcommand{\noi}{\noindent}
\newcommand{\prob}[1]{\vspace{.2in} \noindent {\bf Problem #1.}\\}
\newcommand{\subprob}[1]{ \vspace{.2in} \noindent {\bf #1.}\\}


%Plain eps or pdf figure. Use IPE to embed tex in it.
\newcommand{\fig}[2][1.0]{
  \begin{center}
    \includegraphics[scale=#1]{#2}
  \end{center}}
%Combined PS/Latex figure. This is option of choice for including tex
%code from xfig. Remember to export from xfig using "combined ps/latex" option
\newcommand{\figpst}[2][0.8]{
  \begin{center}
    \resizebox{#1\textwidth}{!}{\input{#2.pstex_t}}
  \end{center}}
%Combined PDF/Latex figure. This is option of choice for including tex
%code from xfig. Remember to export from xfig using "combined pdf/latex" option
\newcommand{\figpdft}[2][0.8]{
  \begin{center}
    \resizebox{#1\textwidth}{!}{\input{#2.pdf_t}}
  \end{center}}



%Algorithmic Environment stuff
\newcommand{\INPUT}{\item[\textbf{Input:}]}
\newcommand{\OUTPUT}{\item[\textbf{Output:}]}
\newcommand{\PARAMETER}{\item[\textbf{Parameter:}]}


%LP environment stuff
\newcommand{\mini}[1]{\mbox{minimize} & {#1} &\\}
\newcommand{\maxi}[1]{\mbox{maximize} & {#1 } & \\}
\newcommand{\maxis}[1]{\mbox{max} & {#1 } & \\}
\newcommand{\minis}[1]{\mbox{min} & {#1 } & \\}
\newcommand{\find}[1]{\mbox{find} & {#1 } & \\}
\newcommand{\st}{\mbox{subject to} }
\newcommand{\sts}{\mbox{s.t.} }
\newcommand{\con}[1]{&#1 & \\}
\newcommand{\qcon}[2]{&#1, & \mbox{for } #2.  \\}
\newenvironment{lp}{\begin{equation}  \begin{array}{lll}}{\end{array}\end{equation} }
\newenvironment{lp*}{\begin{equation*}  \begin{array}{lll}}{\end{array}\end{equation*}}




%% MISC





==> backup - Copy/model.tex <==
\section{Preliminaries}

% We model the problem of pricing against a deceptive buyer as a Stackelberg game (SG) between a leader (seller, she) and a follower (buyer, he). 

\paragraph{Basic Setup of the Optimal Pricing Problem.} A seller (\emph{she}) would like to  sell $d$ different types of \emph{divisible} goods to a buyer (\emph{he}).  It costs her $c(\bvec{x})$ to produce $\bvec{x} \in \RR^d$ bundle of these goods. Let $X \subset \RR^d$ denote the set of all  feasible bundles  that the seller can produce.  We assume $X$ is convex, closed and has positive measure. As a standard assumption  \cite{mas1995microeconomic,roth2016watch,beigman2006learning,balcan2014learning,zadimoghaddam2012efficiently}, the buyer has a \emph{concave} value function $v(\bvec{x})$  for any goods bundle $\bvec{x} \in X$. We do not make any assumption about the seller's production cost   $c(\bvec{x})$, except that it  is monotone non-decreasing.  For normalization, we assume $\bvec{0} \in X$ and $v(\bvec{0} ) = c(\bvec{0} ) =0$.  % Our results do not rely on any other assumptions about $c(\bvec{x})$ and $v(\bvec{x})$. We will show how the shape of $c(\bvec{x})$ affects our conclusions.  % We use $G(c, v)$ to denote the SG played by the seller with cost function $c(\bvec{x})$ and the buyer with value function $v(\bvec{x} )$

The seller aims to find a revenue-maximizing  pricing scheme  assuming rational buyer behaviors. A seller pricing scheme is a function $p(\bvec{x})$ that specifies the sale price for any bundle $\bvec{x}$. By convention,  $p(\bvec{0}) = 0$ always.  Let the set $\P$ denote the set of all pricing \emph{functions} that are allowed to use by the buyer.  The majority of this paper will  focus on the textbook-style \emph{linear} pricing scheme  \cite{mas1995microeconomic}. A linear pricing scheme is parameterized by a price vector $\bvec{p} $ (to be designed) such that $p (\bvec{x})= \bvec{p} \cdot \bvec{x}$ where $i$'th entry $p_i$   is interpreted as the unit price for goods $i$.   Let set \[\P_L = \{p: p(\bvec{x}) = \bvec{p} \cdot \bvec{x} \text{ for some } \bvec{p}   \in \mathbb{R}^d_{+} \}\]  denote the set of all linear pricing functions.  In Section \ref{sec:nonlinear-pricing} we will  also study the  broader classes of \emph{concave} pricing schemes where the set $\P$  consists  of  all  monotone non-decreasing concave  functions. 

 For any price function   $p \in \P$, a rational buyer looks to purchase bundle $\bvec{x}^*$ that maximizes his \emph{utility}; That is, $\bvec{x}^* = \arg \max_{\bvec{x} \in X} \big[ v(\bvec{x}) - p( \bvec{x})  \big]$. Ties are  broken in favor of the seller.\footnote{This is usually without loss of generality since the seller can always induce desirable tie breaking by providing a negligible additional incentive  to the buyer.}
The buyer's best response can thus be viewed as a function  $\bvec{x}^*(p)$ of the seller's price function $p(\bvec{x})$. Knowing that the buyer will best respond, the seller would like to pick the pricing function  $p^* \in \P$ to maximize her revenue. Formally, $p^*$ is the solution to the following bi-level optimization:
% \footnote{
% The optimal solution to such a bi-level optimization problem is called the \emph{Strong Stackelberg equilibrium} (SSE) \cite{roth2016watch}. We shall call $\bvec{p}^*$ the SSE price and $\bvec{x}^*$ the SSE bundle. 
%defined formally as follows %However, it is typically more convenient to view the pricing problem from the perspective of \emph{mechanism design} instead of equilibrium computation. }     
% \vspace{-4mm}
\begin{equation}\label{eq:opt-price}
	p^* = \argmax_{p \in \P}  [  p( \bvec{x}^*(p))  - c(\bvec{x}^*(p)) ],   \quad \text{ where }\,  \bvec{x}^*(p) = \argmax_{\bvec{x} \in X} \big[ v(\bvec{x}) - p( \bvec{x} ) \big] 
\end{equation}
The optimal solution $\big(p^*, \bvec{x}^*(p^*)\big)$ to such a bi-level optimization problem forms an \emph{equilibrium} of this pricing game.  More formally, this is often called the \emph{optimal}  Stackelberg equilibrium or  \emph{strong} Stackelberg equilibrium  \cite{conitzer2006computing,roth2016watch}. We   call $p^*$ the \emph{equilibrium pricing function} and $\bvec{x}^*$ the \emph{equilibrium bundle}.  Note that this is a challenging \emph{functional} optimization problem since the seller is picking a function $p \in \P$, while not a vector variable. However, when $\P = \P_L$ is the set of linear pricing scheme, the above problem becomes a bi-level variable  optimization problem since any $p(\bvec{x}) \in \P_L$ can be fully characterized by a price vector $\bvec{p}$. 

%When the pricing function  $p (\bvec{x})$ can be a general function, Formulation \ref{eq:opt-price} remains the same, except for $ \bvec{p} \cdot \bvec{x}$ being substituted by function $p (\bvec{x})$. 

{\bf Terminologies from Convex Analysis. } We defer basic definitions like convex/concave functions and super/sub-gradients to Appendix \ref{app_sec:convex_background}, and only mention two useful notations here: (1) the set of super/sub-gradient for concave/convex function $f$ is denoted as $\partial f(\mathbf{x})$;  (2)  The  \emph{Bregman divergence} of a function $f$ is defined as   $D_{f}(\mathbf{z},\mathbf{x}) = f(\mathbf{z}) - f(\mathbf{x}) - \nabla f(\mathbf{x})\cdot [  \mathbf{z}- \mathbf{x}]$. $D_{f}(\mathbf{z},\mathbf{x})$ is an important distance notion and is strictly positive for strictly convex functions when  $\mathbf{z} \not = \mathbf{x}$.    



\section{A Model of \texttt{P}ricing \texttt{A}gainst a \texttt{D}eceptive  Buyer in the \texttt{D}ark (\name) }\label{sec:model}
%One crucial issue in the above  pricing problem    is that the seller  needs to know the buyer's value function $v(\bvec{x})$ in order to compute her optimal price function $p^*$.  
%However,  in most realistic situations, the seller does not know buyers' values.  This naturally gives rise to a learning question: how can the seller learn the optimal  pricing scheme from the data generated by interacting with the buyer?  Unsurprisingly, this natural learning question  has received much recent attention. For example, a series of works have demonstrated how the seller can learn the welfare-optimal or revenue-optimal prices by repeatedly  posting ``probing" prices and gradually learn the optimal price from  buyer's purchase responses, a.k.a., the \emph{revealed preferences} \cite{amin2015online,roth2016watch,roth2020multidimensional}.  


%The design of those price learning algorithms is \emph{not} our focus here, but they motivated this work. Specifically, we seek to understand to what extent   these learning algorithms can learn the optimal prices. One crucial challenge of learning to price against a buyer,  compared for example to  learning to  recognize images or  audio,  is that the buyer is naturally a strategic and self-interested agent.  Therefore, a buyer   would have incentives to manipulate or even deceive  the  learning algorithm in order to induce a price that he favors.  As we will show later, a robust manipulation strategy for the buyer is actually not too difficult to figure out.   


As mentioned in related work section \ref{sec:related}, the literature of  algorithms to learn pricing schemes from unknown buyers is massive. This work, however, takes a different perspective and seeks to understand how a buyer can strategically deceive the seller, through a simple yet effective class of manipulation strategies.  
Our model naturally captures a buyer's strategic responses to seller's pricing algorithms  when the seller has no prior knowledge about the buyer, i.e.,    pricing ``in the dark''.  

%To focus our attention on the strategic aspects of the problem, we abstract out the learning procedure  and 
%\mh{We consider a seller who commits to using any optimal pricing scheme with respect to the unknown buyer.} 
Thus, we study a buyer manipulation strategy that is  \emph{oblivious} to   any  pricing algorithm. That is, the buyer simply imitates a different   value function $u(\bvec{x})$ by consistently responding to \emph{any} seller acts  according to $u(\bvec{x})$. Consequently, whatever the seller learns will be with respect to this \emph{imitative value function} $u(\bvec{x})$.  Alternatively, one can think of the buyer as  \emph{committing} to always behave   according to   value function $u(\bvec{x})$. Nevertheless, the buyer's objective is still to maximize his \emph{true} utility by carefully crafting an imitative  value function $u(\bvec{x})$ to commit to. Given   the buye's commitment to  value function $u(\bvec{x})$, the best pricing scheme for  the seller is to use the optimal pricing function against buyer value function $u(\bvec{x})$.  Similar to $v(\bvec{x})$, the imitative value functions $u(\bvec{x})$ is  assumed to be concave and monotone non-decreasing as well. Let set $\C$ denote the set of all such functions. These  resulted in the following model of  \emph{Pricing Against a Deceptive buyer in the Dark} (\name{}): 
	\begin{itemize} 
		\item  The buyer with true value function $v(\bvec{x})$ (unknown to seller) commits to react optimally according to an \emph{imitative value function} $u(\bvec{x}) \in 		\C$. 
		\item  The seller learns the buyer's imitative value function $u(\bvec{x})$ and compute the optimal pricing function $p^* \in \P$ by solving bi-level Optimization Problem \eqref{eq:opt-price} w.r.t. $u(\bvec{x})$. 
		\item The buyer observes the seller's pricing function $p^*$, and then follows his commitment to react optimally w.r.t. to $u(\bvec{x})$ by purchasing bundle $\bvec{x}^* = \arg\max_{\bvec{x} \in X} [ u(\bvec{x}) - p( \bvec{x})]$. 
	\end{itemize}
 %\footnote{  Without the buyer's commitment assumption, the seller's pricing  and the buyer's value imitation will happen simultaneously. That will lead to a different, simultaneous-move, game model.}  
 We remark that such  commitment to a fake value function is not uncommon  in the literature; similar assumptions have been adopted in many recent works in, e.g., auctions \cite{tang2018price}, general Stackelberg games \cite{gan2019imitative,birmpas2020optimally} and security games \cite{gan2019manipulating,nguyen2019imitative,nguyen2020decoding}.  The buyer's ability of making such a commitment  fundamentally comes from the fact that the seller has no prior knowledge about the buyer's true value function $v(\bvec{x})$, i.e., has to ``price in the dark''. We refer curious reader to  Appendix \ref{app_sec:commitment} for a more  detailed discussion about  this assumption. 
 
 Naturally,   the buyer  with true value function $v(\bvec{x})$  would like to find the optimal imitative value function $u^*(\bvec{x})$  to maximizes his utility. This results in the following  equilibrium definition. 
\begin{definition}[Equilibrium of \name]\label{def:equ}
The equilibrium of \name{} consists of the optimal imitative value \emph{function} $u^* \in \C $ that the buyer  commits to, the seller's optimal pricing function $p^* \in \P$  against $u^*(\bvec{x})$, and the buyer's response bundle $\bvec{x}^*\in X$. Formally,  $(u^*, p^*, \bvec{x}^*)$ is an equilibrium for a buyer with true value function $v(\bvec{x})$ to \name{} if 
\begin{eqnarray}\nonumber 
 u^* = \argmax_{u  \in \C}  [  v(\bvec{x}^*) - p^*(\bvec{x}^* ) ], \qquad   
 \text{ where } &&   p^* = \argmax_{p \in \P}  [  p( \bvec{x}^*)  - c(\bvec{x}^*) ],   \\ \label{eq:equilibrium-def} 
 \text{ where }  &&  \bvec{x}^* = \argmax_{\bvec{x} \in X} \big[ u^*(\bvec{x}) - p^*( \bvec{x} ) \big]. 
\end{eqnarray} 
 \vspace{-4mm}
\end{definition}
The equilibrium of \name{} gives rise to  a challenging \emph{tri-level functional optimization problem}.\footnote{Even for linear pricing where $\P = \P_L$, this is still a functional optimization problem since the buyer's imitative value function $u$ is an arbitrary function in $\C$. } Note that, the dependence of the buyer's objective $[  v(\bvec{x}^*) - p^*(\bvec{x}^* ) ]$ on $u$ is indirectly through the two argmax problems afterwards.  The buyer is assumed to  know the production cost function $c(\bvec{x})$, which is needed to compute his optimal $u^*$. This can be easily justified in situations where the seller has been on the market for some time, therefore her production cost gradually becomes public knowledge. 





